Decompose, Compare, and Decide: Multimodal LLMs are Implicit Few-Shot Learners

Multimodal Large Language Models (MLLMs) have demonstrated remarkable abilities when analyzing images, yet translating these capabilities to few-shot image classification remains challenging. To bridge this gap, we present DeCoDe, a simple yet effective technique that enables off-the-shelf MLLMs to act as strong few-shot classifiers without any additional training. Our approach builds on the idea of few-shot classification as a set of pairwise image comparisons, decomposing the task into a set of binary decisions. Given a query image and a support image from a candidate class, the MLLM is prompted to decide whether the two images depict the same class. The logit corresponding to an affirmative response is then used as a similarity score to assign the query image to the most likely class. While this already yields good results, we show that providing additional high-level information, such as the data domain, to the model further improves performance. Our evaluation provides an extensive analysis of various inference variants on a suite of twelve datasets, six established and six newly curated few-shot benchmarks spanning across diverse domains. The results show that the proposed simple decomposition technique can turn off-the-shelf MLLMs into powerful few-shot learners, significantly outperforming current state-of-the-art few-shot methods on both standard and novel domains. Code is available at https://github.com/yunhanwang1105/DeCoDe.

==> ECCV_2026/preamble.tex <==
% ---------------------------------------------------------------
% Other packages

% Commonly used abbreviations (\eg, \ie, \etc, \cf, \etal, etc.)
\usepackage{eccvabbrv}

% Include other packages here, before hyperref.
\usepackage{graphicx}
\usepackage{booktabs}

% The "axessiblity" package can be found at: https://ctan.org/pkg/axessibility?lang=en
\usepackage[accsupp]{axessibility}  % Improves PDF readability for those with disabilities.


% ---------------------------------------------------------------
% Hyperref package

% It is strongly recommended to use hyperref, especially for the review version.
% Please disable hyperref *only* if you encounter grave issues.
% hyperref with option pagebackref eases the reviewers' job, but should be disabled for the final version.
%
% If you comment hyperref and then uncomment it, you should delete
% main.aux before re-running LaTeX.
% (Or just hit 'q' on the first LaTeX run, let it finish, and you
%  should be clear).

% TODO FINAL: Comment out the following line for the camera-ready version
%\usepackage[pagebackref,breaklinks,colorlinks,citecolor=eccvblue]{hyperref}
% TODO FINAL: Un-comment the following line for the camera-ready version
\usepackage{hyperref}

% Support for ORCID icon
\usepackage{orcidlink}

\usepackage{multirow}
\usepackage{booktabs}
\usepackage{tabularx}
\usepackage{array}
\usepackage{colortbl,xcolor,adjustbox}
\usepackage{float}
\usepackage{wrapfig}

% For check mark
\usepackage{amssymb}% http://ctan.org/pkg/amssymb
\usepackage{pifont}% http://ctan.org/pkg/pifont
\usepackage{soul}
\usepackage{placeins}
\usepackage{makecell}

%% ---- Colour palette -----------------------------------------------
% Header bands
\definecolor{stdblue}{RGB}{207,222,243}      % standard datasets header
\definecolor{novelamber}{RGB}{252,228,190}   % novel datasets header

% Section rows
\definecolor{secblue}{RGB}{232,240,252}      % semantic section bg
\definecolor{secorange}{RGB}{255,243,224}    % anonymous section bg
% Best / second-best cell highlights
\definecolor{gold}{RGB}{255,215,0}           % 1st best
\definecolor{silver}{RGB}{210,210,210}       % 2nd best
% Rank colours for text
\definecolor{rankone}{RGB}{180,0,0}          % deep red = best
\definecolor{ranktwo}{RGB}{0,100,160}        % steel blue = 2nd
% Model sub-header tint
\definecolor{modeltint}{RGB}{245,245,245}

\definecolor{woodbrown}{RGB}{92,51,23}

\definecolor{almond}{rgb}{0.98, 0.95, 0.93} % highlight table
\definecolor{lightgreenrow}{rgb}{0.92, 0.97, 0.92}
\definecolor{lightredrow}{rgb}{0.98, 0.92, 0.92}

\newcommand{\best}[1]{\cellcolor{gold}\textbf{\textcolor{rankone}{#1}}}
\newcommand{\second}[1]{\cellcolor{silver}\textbf{\textcolor{ranktwo}{#1}}}


\newcommand{\xmark}{\ding{55}} % cross mark
\newcommand{\cmark}{\ding{51}} % check mark 

% Please change as per preferences
\newcommand{\hkc}[1]{{\color{blue} {\bf HK:} #1}}
\newcommand{\YW}[1]{{\color{magenta} {\bf YW:} #1}}
\newcommand{\EK}[1]{{\color{purple} {\bf EK:} #1}}
\newcommand{\WB}[1]{\textcolor{cyan}{\bf WB: #1}}
\newcommand{\EA}[1]{{\color{orange} {\bf EA:} #1}}
\newcommand{\NS}[1]{{\color{green!50!black} {\bf NS:} #1}}

\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\draftfig}[1]{\fbox{\parbox[c][8cm][c]{\linewidth}{#1}}} % placeholder figure

\usepackage[most]{tcolorbox}
\newtcolorbox{promptbox}[1][]{%
  enhanced,
  boxrule=0.4pt,
  colback=black!2,
  colframe=black!25,
  arc=2pt,
  left=6pt,right=6pt,top=6pt,bottom=6pt,
  fontupper=\footnotesize\ttfamily,
  #1
}

\usepackage{caption}

\captionsetup[figure]{font=small,labelfont=bf}

==> sec/0_abstract.tex <==
\begin{abstract}


Multimodal Large Language Models (MLLMs) have demonstrated remarkable abilities when analyzing images, yet translating these capabilities to few-shot image classification remains challenging. To bridge this gap, we present DeCoDe, a simple yet effective technique that enables off-the-shelf MLLMs to act as strong few-shot classifiers without any additional training.
Our approach builds on the idea of few-shot classification as a set of pairwise image comparisons, decomposing the task into a set of binary decisions. 
Given a query image and a support image from a candidate class, the MLLM is prompted to decide whether the two images depict the same class.
The logit corresponding to an affirmative response is then used as a similarity score to assign the query image to the most likely class.
While this already yields good results, we show that providing additional high-level information, such as the data domain, to the model further improves performance.
Our evaluation provides an extensive analysis of various inference variants on a suite of twelve datasets, six established and six newly curated few-shot benchmarks spanning across diverse domains. The results show that the proposed simple decomposition technique can turn off-the-shelf MLLMs into powerful few-shot learners, significantly outperforming current state-of-the-art few-shot methods on both standard and novel domains. Code is available at \url{https://github.com/yunhanwang1105/DeCoDe}.

\keywords{Few-Shot Learning \and Multimodal Large Language Models \and Vision-Language Models \and In-Context Learning}

% consistently

% Multimodal large language models (MLLMs) have demonstrated remarkable success in vision–language problems such as VQA and captioning, yet their capabilities have not so far transferred to few-shot visual recognition. \NS{another version: Multimodal large language models (MLLMs) have demonstrated remarkable reasoning abilities when analyzing images, e.g., answering complex visual queries and producing detailed descriptions, yet translating their capabilities to few-shot visual classification remains challenging.} To bridge this gap, we present a simple, training-free technique that leverages MLLMs as implicit few-shot learners without any additional training or adaptation. \NS{another: In this work, we present a simple yet effective technique that enables off-the-shelf MLLMs to act as strong few-shot classifiers without any additional training or adaptation.}
% Our approach picks up on the idea of few-shot classification as a sequence of pairwise image comparisons, decomposing the few-shot task into a set of binary decisions. Given a query image and a support image \NS{from a candidate class}, the MLLM is prompted to decide whether the two depict the same or different classes. 
% We then extract the logits of the corresponding answer tokens  and use them \NS{the log-likelihood of affirmative response and use it} as similarity scores to assign the query image to its most likely support class image. 
% We provide a thorough analysis of various inference variants on a suite of twelve datasets, six established and six new few-shot datasets spanning diverse visual domains, showing that the proposed decomposition allows off-the-shelf MLLMs to capture visual similarity  to act as strong, implicit few-shot learners and that they can consistently outperform current state-of-the-art few-shot methods across a range of tasks and domains. \NS{.. showing that the proposed simple decomposition enables MLLMs to serve as competitive implicit few-shot learners, consistently outperforming current state-of-the-art few-shot methods across a wide range of tasks and domains. Should we add some numbers here?} 


% Large multimodal language models (MLLMs) exhibit strong zero-shot visual recognition, yet their few-shot performance remains inconsistent. We identify a counterintuitive phenomenon: on benchmarks well-aligned with pretraining, one-shot prompting can match or underperform zero-shot inference — a failure mode we term semantic dominance, where prior alignment to canonical class names overwhelms in-context visual supervision. On semantically novel datasets, however, one-shot prompting surpasses zero-shot baselines, revealing latent few-shot capacity sensitive to inference design. An anonymized evaluation replacing class names with abstract identifiers confirms that current pipelines rely heavily on semantic labels rather than support–query visual correspondence. Motivated by this analysis, we propose FS-DEMMO, a training-free framework that reformulates N-way classification into structured pairwise binary comparisons, directly mitigating semantic dominance while unlocking the implicit few-shot learning capacity of pretrained MLLMs. FS-DEMMO is model-agnostic and requires no fine-tuning. Experiments across pretraining-aligned and semantically novel benchmarks achieve an 88.0\% total average accuracy — a +10.7 point gain over the prior best — with a +16.5 point increase on novel categories (76.9\% vs. 60.4\%).

\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{ECCV_2026/figures/teaser_figure.pdf}
\caption{
We propose a decomposed prompting technique (DeCoDe) for few-shot classification with MLLMs. We \textbf{decompose} the task into pairwise support–query comparisons, asking whether two images belong to the same class. 
By ranking the model’s affirmative responses across candidate pairs (\textbf{compare}) and selecting the highest-scoring logit as the predicted class (\textbf{decide}), MLLMs become strong few-shot classifiers without any training. Unlike standard in-context prompting, which relies heavily on semantic label names, our decomposed approach succeeds even with anonymized labels by forcing the model to perform direct visual-to-visual comparison. 
}
\label{fig:teaser}
\end{figure}

% what is FSL - can shift to intro/remove
% Few-shot learning (FSL) enables generalization to new tasks using limited labeled examples, making it suitable for real-world scenarios where large annotated data is unavailable or adaptation to novel tasks is required at inference time.
% In the standard \textit{N-way K-shot} setting, models classify a query image into one of N classes given K labeled examples per class. \NS{<-- I don't think it's needed} The first few-shot methods achieved this by training a model on a set of base classes and then testing it on a held-out set of novel classes~\cite{vinyals2016matching, snell2017prototypical, finn2017model, sung2018learning, ravi2017optimization}. With the emergence of foundation models that were trained on large-scale web data via self- or weakly-supervised contrastive methods such as DINO~\cite{oquab2023dinov2} and CLIP~\cite{lpclip}, the focus shifted towards exploring how the learned representation can be leveraged for better few-shot classification~\cite{chi2025learning, proker, tipadapter, coop, coopop, clipadapter, tian2020rethinking}. Recently, advanced Vision-Language models such as InternVL3~\cite{zhu2025internvl3}, and Qwen3-VL~\cite{bai2025qwen3}, also referred to as Multimodal Large Language Models (MLLMs), have become another strong focus of research. As a result, they were also explored for few-shot learning \cite{liu2024, Yang_2025_Verbalized}.

Few-shot learning (FSL) enables models to generalize to new tasks and domains using only a small number of labeled examples per class. This can be especially valuable for real-world scenarios where large annotated datasets are unavailable or adaptation to novel tasks is required at inference time. Early few-shot methods required model training on a set of base classes in order to enable recognition of held-out novel classes~\cite{vinyals2016matching, snell2017prototypical, finn2017model, sung2018learning, ravi2017optimization, Kukleva_2021_ICCV}. With the emergence of foundation models trained on large-scale web data via self- or weakly-supervised objectives, such as DINO~\cite{oquab2023dinov2} or CLIP~\cite{lpclip}, the focus shifted towards exploring how pretrained representations can be leveraged for improved few-shot classification with minimal or no additional training~\cite{chi2025learning, proker, tipadapter, coop, coopop, clipadapter, tian2020rethinking}. More recently, multimodal large language models (MLLMs), such as LLaVA-OneVision~\cite{li2024llava}, InternVL3~\cite{zhu2025internvl3}, or Qwen3-VL~\cite{bai2025qwen3}, have demonstrated strong vision-language capabilities, raising the question of whether such models can also serve as effective few-shot learners~\cite{liu2024, Yang_2025_Verbalized}.


% \NS{This paragraph is a bit lacking focus now. Do you want to motivate MLLMs for few-shot learning here?} \YW{I think we should mention LLaVA somewhere.}

% This work follows the latter line of research and argues that current MLLMs, trained on a vast amount of web content, are already implicit few-shot learners. 

%This work follows the latter line of research and argues that current MLLMs, trained on a vast amount of web content, already possess implicit few-shot capabilities. 

% So far, MLLMs have been explored for few-shot learning in two ways: via in-context learning by adding all support images together with the query image to a single prompt~\cite{liu2024}, or via transcribing the image first and leveraging the text~\cite{Yang_2025_Verbalized}, or by pairwise comparisons either directly on images followed by a learning pipeline~\cite{liu2024} 

So far, MLLMs have been explored for few-shot learning in three ways: by extracting discriminative embeddings from the internal representations of the MLLM~\cite{sav}, 
% by verbalizing discriminative features through pairwise comparisons and searching for these characteristics in the query image
by verbalizing discriminative visual features and matching them to query images~\cite{Yang_2025_Verbalized}, or via in-context learning where support and query images are jointly provided in a single prompt~\cite{liu2024}. However, in-context prompting has been shown to perform poorly for few-shot image classification when used off-the-shelf~\cite{sav,liu2024}, often requiring additional fine-tuning to encourage stronger reliance on the support examples~\cite{liu2024}. 
% \YW{I think this paper did not do pairwise image match, they had pairwise image-caption match, they still put all information in a single prompt. Or maybe I don't understand this sentence correctly}
% The proposed approach picks up on this idea by decomposing the few-shot task into pairwise binary prompts asking the MLLMs to indicate if two images show the same class or not.
% Different from existing methods, especially~\cite{liu2024, Yang_2025_Verbalized}, we simply use the logit score of the \texttt{Yes} token to rank all pairs and select the highest class.
% The proposed approach builds on the idea of pairwise comparisons and decomposes the few-shot task into binary prompts that ask the MLLM to decide whether two images belong to the same class or not. 

To address this limitation, the proposed approach reformulates few-shot classification as a set of pairwise comparisons. Instead of reasoning over all support examples jointly, the few-shot task is decomposed into binary prompts asking the MLLM whether a query image and a support image belong to the same class.
Unlike existing methods, particularly~\cite{liu2024,Yang_2025_Verbalized}, the proposed technique considers the logit of the \texttt{Yes} token to rank all candidate pairs and assign the query image to the most likely class.
% While this simple technique, when applied to standard MLLMs, is already enough to outperform, it actually shows that MLLMs can further benefit from context information, such as the domain of the data they are given. 
While this simple technique, when applied to standard MLLMs, is already sufficient to outperform current state-of-the-art methods, it shows that the models can benefit from contextual information, such as the domain of the data. 
% Namely, we show that those models further improve when they are given the topic of the dataset, such as car, aircraft, etc. 
Namely, we found that the performance of the pairwise decomposed setting further improves when models are given the topic of the data, usually based on the dataset name, such as cars, yoga poses, etc. 
% We thus coin the respective workflow as \textit{Decompose}, \textit{Compare}, \textit{Decide}, and show that its application can turn current state-of-the-art MLLMs into high-performing few-shot learners. 
We thus coin the respective workflow as \textit{\textbf{De}compose}, \textit{\textbf{Co}mpare}, \textit{\textbf{De}cide} (DeCoDe) and show that this technique can transform state-of-the-art MLLMs into high-performing few-shot learners. 


% One problem with the evaluation of web-scale trained models and backbones for few-shot tasks is that their performance is therefore likely influenced by potential overlap between benchmark datasets and the pretraining corpora of VLMs and can drop significantly when models must generalize to unseen classes using only the support set, suggesting that models rely on memorized pretraining knowledge rather than adapting to the support examples at inference time~\cite{kravets2025}. 
However, evaluating the few-shot capabilities of web-scale pretrained models remains challenging. In particular, the performance of models on standard few-shot benchmarks may be influenced by potential overlap between benchmark datasets and the models’ pretraining corpora. As a result, models may rely on memorized knowledge rather than adapting to the provided support examples~\cite{kravets2025rethinking}.
To address this issue, we conduct an extensive analysis on two sets of datasets and in two evaluation modes.  \textit{First}, with respect to datasets, we consider six standard few-shot datasets, as well as six novel datasets, which can be considered as out-of-domain for web-scale trained models. 
We observe that most MLLMs already achieve near-perfect accuracy on the standard datasets in a 0-shot setting, often even exceeding 1-shot performance. In contrast, we consider novel, out-of-domain datasets as datasets that show substantially low 0-shot performance as well as a clear improvement from 0-shot to a simple 1-shot baseline. We consider this as an indication that the model might have seen less of the original data and needs to rely more on visual cues.
% \textit{Second}, we consider two different few-shot settings for MLLMs, first the case where the semantic class labels of the support set are given to the model together with the support image, as well as a second scenario, where either no class names are given, or the class names are anonymized, e.g., in case of in-context learning support images are just labeled by a numerical index such as \texttt{Class 1, Class 2, etc.}.
% In this case, the model can not directly rely on textual knowledge, as it needs to connect the visual representation of the query image to the support images. 
\textit{Second}, we consider two different few-shot settings for MLLMs: first, we consider a semantic setting, in which semantically meaningful class labels are provided together with the support images, and, second, we consider an anonymized setting, where support images are labeled only with numerical identifiers (e.g., \texttt{Class 1}, \texttt{Class 2}), preventing the model from relying directly on textual knowledge.
Our analysis shows that the anonymization alone is enough to reduce the performance of MLLMs for in-context learning, even on standard benchmarks, whereas the proposed decomposition is able to significantly increase the performance in all cases, with and without class labels, as well as for standard and novel datasets.  
% Overall, we show that in the proposed setting, current MLLMs can be considered as highly performative few-shot learners.


%
The contributions of this work can be summarized as follows: 
\begin{itemize}
    \item We propose a simple, yet effective technique of \textit{Decompose, Compare, Decide} (DeCoDe), to turn MLLMs into powerful few-shot learners by ranking the logits corresponding to an affirmative response to a binary prompt question. 
    \item We show that decomposed MLLMs can further benefit from high-level cues such as domain information and propose a new few-shot evaluation scenario by providing the global dataset domain as context. 
    % \item We provide an extensive evaluation of current MLLMs for few-shot learning, showing that out-of-domain data still allows to assess the real few-shot capabilities of those models. 
    \item We conduct a systematic evaluation of current MLLMs for few-shot learning across standard and novel out-of-domain datasets and under different modes, including anonymized class labels, revealing when models rely on memorized pretraining knowledge versus true few-shot adaptation.
    % The analysis highlights the impact of dataset overlap with pretraining data and reveals when models rely on memorized knowledge versus true few-shot adaptation.
\end{itemize}

% \hkc{We might need a nice overview figure if we have a bit of space ... things we might want to explain are standard/novel datasets and w/wo labels OR the different settings: in context vs pairwise prompting ... }


==> sec/2_relwork.tex <==
\section{Related Works}
\label{sec:relwork}

% \paragraph{Classical Few-Shot Methods:}

% \hkc{Not sure if we really need this ... } \YW{We can write some if we have space later.}

\paragraph{VLM Embeddings for Few-Shot Learning.}

Vision-Language Models (VLMs) such as CLIP provide a strong foundation for FSL by enabling classification based on embedding similarity.
Prior work has adapted such embeddings for few-shot tasks via prompt learning~\cite{coop, coopop, prograd, kgcoop, plot, maple} or adapter-based methods~\cite{clipadapter, taskres, susx, tipadapter}. 
More recent works explore additional adaptation strategies. Two-Stage Few-Shot (2SFS)~\cite{2SFS} performs two-stage PEFT-based representation learning; Logit Deconfusion ~\cite{ldc} addresses class bias at the logit level; ProKeR~\cite{proker} applies training-free kernel regression over pretrained CLIP features; LoRA Recycle~\cite{recyclelora} enables tuning-free adaptation via reuse of pre-trained LoRAs \cite{hu2022lora}. CAML~\cite{fifty2023context} is a large-scale, meta-trained framework built on a ViT \cite{dosovitskiy2020image} backbone that enables in-context classification using frozen image embeddings. 
Unlike methods that modify pretrained encoders, our proposed technique does not adapt the underlying representation or update parameters. Instead, we investigate how frozen MLLMs can perform few-shot classification purely through structured inference.

Finally, Kravets et al.~\cite{kravets2025rethinking} discuss the problem that standard CLIP few-shot evaluations are partially transductive due to pretraining overlap, and introduce an unlearning-based pipeline to construct inductive benchmarks that reveal substantial performance drops in existing methods.
We follow this idea, but instead of unlearning and thus changing the model parameters, we use alternative datasets that can be considered more out-of-domain for web-trained multimodal models. 

\paragraph{MLLMs for Few-Shot Learning.}

Beyond adapting pretrained VLM encoders, SAVs~\cite{sav} extracts representations from MLLMs for downstream few-shot classification. VRL~\cite{Yang_2025_Verbalized} leverages MLLMs to automatically derive interpretable verbalized features that capture inter-class differences and intra-class commonalities. 
Other works explore generative few-shot prompting with MLLMs~\cite{liu2024, sav}, yet such models often remain less effective with respect to embedding-based few-shot methods, despite strong performance on open-ended vision–language tasks. 
A central challenge is their reliance on semantic language priors rather than visual evidence from the support set~\cite{baldassini2024}. GFSL~\cite{liu2024} addresses this in part through label anonymization, applied within a fine-tuning strategy. Across these works, evaluations vary considerably in scope: SAVs focus on standard benchmarks, VRL reports results on novel out-of-domain datasets. Building on this idea, we jointly examine zero-shot and few-shot regimes, the effect of semantic versus anonymized labels, and evaluate across both standard and novel datasets, providing a unified evaluation across these axes. 

% Existing approaches address this issue only partially. GFSL~\cite{liu2024} introduces anonymization, but primarily as part of a fine-tuning strategy rather than as a controlled evaluation tool; moreover, it neither reports zero-shot performance nor evaluates on novel datasets. SAV~\cite{sav} includes zero-shot comparisons but restricts experiments to standard benchmarks. VRL~\cite{Yang_2025_Verbalized} reports few-shot results on out-of-domain datasets, yet does not analyze performance on classical benchmarks or report zero-shot results. Thus, prior work does not provide a unified investigation of (i) zero-shot vs. few-shot behavior, (ii) semantic vs. anonymized labels, and (iii) standard vs. novel domains within a single consistent framework.



==> sec/3_method.tex <==
\section{Method}
\label{sec:method}
% \EK{should we change the section name to 'Inference Framework' or something like that since we don't say method anywhere anymore, or is it fine? }
In this section, we introduce our inference framework for few-shot classification. 
%
~\cref{fig:teaser} illustrates the inference pipeline of our framework.
Given multimodal context consisting of images and text, the MLLM is prompted to predict the class of a query image based on the provided support examples.
Depending on the prompting paradigm, the prediction is either obtained directly from the model's generated response or derived from the model's output logits for specific answer tokens (e.g., `Yes').
% in the decomposed pairwise prompting setting.

% % < ----------------- NEW: Inference Variants: core text -------------->
% \subsection{Inference Variants}
% \label{sec:implementation_InferenceVariants}


~\Cref{tab:variants} summarizes the inference variants evaluated in this work. 
The variants differ along three dimensions: 
(i) the prompting paradigm (in-context learning vs.\ decomposed pairwise prompting);
(ii) the use of dataset-level domain information; and
(iii) the anonymization of semantic class labels.
% Overall, we consider three different variations for inference: (i) first,  we consider in-context learning vs. decomposed prompting; (ii) second, we differentiate between settings with semantic class labels given for each support image vs the anonymized setting without class labels; and (iii) third, we consider the setting where context is given in form of the overall domain information of the dataset.
% \hkc{Could someone double check if the wording in that table is consistent with what we write in the text as well as with the wording for all tables in the Eval section?}
% We further consider the 0-shot in-context performance as a baseline to assess if the model would be able to classify a query based on given knowledge and without visual cues. An overview of the different variants is given in Tab.~\ref{tab:variants}. 
In addition, we evaluate a 0-shot setting as a baseline to assess whether the models can classify a query based solely on its prior knowledge without visual support examples.
% \WB{Do we need the "in-context" in  "0-shot in-context"?}
% \EK{move to later}
In all experiments, we follow the prompt design of~\cite{liu2024} and explore more prompt options in the supplementary material. 
% \NS{maybe move this sentence for later?}
% \EK{mention that refer to fig1 for prompts. prompt exploration in supplement}

% ~\cref{fig:prompts} illustrates the prompt formats used across the different settings described in~\cref{subsec:incontext,subsec:decomposition,subsec:domain,subsec:labels}.

% In the following, we first present the problem formulation (\cref{subsec:problem_formulation}).
% Next, we describe the different variants, including in-context prompting (\cref{subsec:incontext}), decomposed pairwise prompting (\cref{subsec:decomposition}),
% use of dataset-level domain information (\cref{subsec:domain}) and class label anonymization (\cref{subsec:labels}). 
% Finally, we detail the episode construction used for evaluation (\cref{subsec:episodes}).

% \paragraph{Problem Setup.}
% Notations fixes
% 1. Overloaded index in the support set 
% x_i^s -> x_{n,k} |  k-th support image of class c_n +  I also drop the superscript s as the double index already distinguishes support imgs from queries, keeping symbols lighter.

% 2. y_j not defined --> explicitly types y_j as an index and add the subscript j to \hat{y} so the prediction is tied to a specific query.

% 3. \hat{y} and y --> subscript j to match Fix 2.
% 4. In P(i \mid x^q, \mathcal{S}) uses i as both the random variable and the option index + x^q lacks the subscript. --> replace index with n

%  5. Pairwise score is described in words not formula

% 6. other not defined variables M, q in x_j^q, e in Q_e, P

%  Structures fixes:
%  \subsection{Unified Episodic Prompting} was to thin (3 sentences) --> too litle for a whole subsection
% Fix: have 3 subsections: \subsection{Problem Formulation} \subsection{Inference Framework}  \subsection{Inference Variants}  


%%< ----------------- old:method intro -------------->
% We evaluate few-shot classification tasks structured as episodes, where only a few labeled examples per class are available, and the test data may come from a different visual domain than the pretraining data.
% In each episode, an $N$-way label set is sampled,
% \[
% \mathcal{C} = \{c_1, \dots, c_N\},
% \]
% with support set
% \[
% \mathcal{S} = \{(x_i^s, c_i)\}_{i=1}^{N \times K}
% \]
% ($K$ shots per class), and query set
% \[
% \mathcal{Q} = \{(x_j^q, y_j)\}_{j=1}^{M}.
% \]
% Given $(\mathcal{S}, x^q)$, the model predicts $\hat{y} \in \{1, \dots, N\}$.
% Performance is measured by mean episodic accuracy over a set of evaluation episodes $\mathcal{E}$:
% \[
% \mathrm{Acc}
% =
% \frac{1}{|\mathcal{E}|}
% \sum_{e \in \mathcal{E}}
% \frac{1}{|\mathcal{Q}_e|}
% \sum_{(x^q, y) \in \mathcal{Q}_e}
% \mathbf{1}[\hat{y} = y].
% \]

%</ ----------------- old:method intro --------------/>



\subsection{Problem Formulation}
\label{subsec:problem_formulation}

Classical few-shot learning protocols~\cite{vinyals2016matching, snell2017prototypical, finn2017model} divide a dataset into 
% disjoint subsets: 
a set of base classes used for supervised pre-training and a set of novel classes reserved for few-shot evaluation.
In contrast, training-free 
% few-shot learning 
approaches 
% built \EK{was not sure what built here meant}
leverage
VLMs and MLLMs~\cite{tipadapter, susx, sav, proker}, bypassing supervised base-class training, thanks to rich representations acquired during large-scale web pretraining.
In this paper, we follow a training-free protocol in the standard \textit{N-way K-shot} setting. The model's task is to classify a query image into one of $N$ classes given a support set of $K$ labeled examples per class. We define the support set $\mathcal{S}$ to be sampled from the test set as:  
\begin{equation}
\mathcal{S} = \bigl\{(x_{n,k}^s,\, c_n) \mid n=1,\dots,N,\; k=1,\dots,K\bigr\},
\end{equation}
where $N$ is the number of classes sampled, $K$ is the number of samples per class, and  $\mathcal{C} = \{c_1, \dots, c_N\}$ is the set of corresponding class names where each $c_n$ is the semantic name of the $n$-th class.
We formulate the query set~$\mathcal{Q}$ as:
\begin{equation}
\mathcal{Q} = \{(x^q, c_y)\},
\end{equation}
where $x^q$ is the query image and $y \in \{1, \dots, N\}$ is its ground-truth class index with respect to the support classes $\mathcal{C}$.

\input{ECCV_2026/tab/variants}

% \subsection{Overview}
% \label{subsec:overview}
% % \WB{We should add a sentence to frame the paper as an analysis of FS for MLLMs}
% % \NS{Name of the method, D3-FS, is never mentioned in the method section so far, should we introduce it here?}
% % \NS{maybe this might be a new subsection? it's not a problem formulation already, it's method}
% % We treat the MLLM as a black-box predictor.
% % Given multimodal context (images and text), we consider either the text response generated by the MLLM (baseline) or the resulting token-level likelihoods for specific candidate outputs. 
% % \NS{I would add more description here, like what is input/output and so on. Maybe figure as well} 

% ~\cref{fig:teaser} illustrates the inference pipeline of our framework.
% Given multimodal context consisting of images and text, the MLLM is prompted to predict the class of a query image based on the provided support examples.
% Depending on the prompting paradigm, the prediction is either obtained directly from the model's generated response or derived from the model's output logits for specific answer tokens (e.g., `yes').
% % in the decomposed pairwise prompting setting.

% % % < ----------------- NEW: Inference Variants: core text -------------->
% % \subsection{Inference Variants}
% % \label{sec:implementation_InferenceVariants}


% ~\Cref{tab:variants} summarizes the inference variants evaluated in this work. 
% The variants differ along three dimensions: 
% (i) the prompting paradigm (in-context learning vs.\ decomposed pairwise prompting);
% (ii) the use of dataset-level domain information; and
% (iii) the anonymization of semantic class labels.
% % Overall, we consider three different variations for inference: (i) first,  we consider in-context learning vs. decomposed prompting; (ii) second, we differentiate between settings with semantic class labels given for each support image vs the anonymized setting without class labels; and (iii) third, we consider the setting where context is given in form of the overall domain information of the dataset.
% % \hkc{Could someone double check if the wording in that table is consistent with what we write in the text as well as with the wording for all tables in the Eval section?}
% % We further consider the 0-shot in-context performance as a baseline to assess if the model would be able to classify a query based on given knowledge and without visual cues. An overview of the different variants is given in Tab.~\ref{tab:variants}. 
% In addition, we evaluate a 0-shot setting as a baseline to assess whether the models can classify a query based solely on its prior knowledge without visual support examples.
% % \WB{Do we need the "in-context" in  "0-shot in-context"?}
% % \EK{move to later}
% In all experiments, we follow the prompt design of~\cite{liu2024} and explore more prompt options in the supplementary material. 
% % \NS{maybe move this sentence for later?}
% % \EK{mention that refer to fig1 for prompts. prompt exploration in supplement}
% ~\cref{fig:prompts} illustrates the prompt formats used across the different settings described in~\cref{subsec:incontext,subsec:decomposition,subsec:domain,subsec:labels}.

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figures/prompts.pdf}
\caption{
Variants of prompt formulations used in our experiments. 
\textbf{(a)} standard in-context prompting with semantic labels. 
\textbf{(b)} standard in-context prompting with anonymized labels. 
\textbf{(c)} decomposed pairwise prompting with semantic labels. 
\textbf{(d)} decomposed pairwise prompting with anonymized labels.
\textbf{(e)} decomposed pairwise prompting with domain information and semantic labels. 
\textbf{(f)} decomposed pairwise prompting with domain information and anonymized labels.
}
\label{fig:prompts}
\end{figure}

\subsection{In-Context Few-Shot Classification with MLLMs }
\label{subsec:incontext}
To assess the few-shot capabilities of current MLLMs, we consider few-shot learning as an in-context learning task.
% , where the model is first shown the set of support images together with the respective class label, and then the query image together with the respective class options. 
% The model is first shown the support images together with their corresponding class labels, followed by the query image and a list of candidate class options.
% Namely, 
% Given the support set and a query image, $(\mathcal{S}, x^q)$, we prompt an MLLM to predict the class of a query image via multiple choice selection as it provides good instruction following capabilities and most models can be assumed to do well on this task.
Given a support set $\mathcal{S}$ and a query image $x^q$, the model is prompted to predict the class of the query image via multiple-choice selection over the candidate classes.
The prompt consists of the concatenation of all support images with their corresponding class labels, followed by the query image and the list of candidate class options.
% The respective prompt is the concatenation of all support images with their respective class information and the query image. 
The resulting prompt $p$ is structured as: 
\begin{equation}
p = x^s_{1,1} \oplus \texttt{Str} \oplus c_1 \dots x^s_{N,K} \oplus \texttt{Str} \oplus c_N\ \oplus  \\
x^q \oplus \texttt{Str} \oplus 1. \, c_1; 2. \, c_2; \dots ;  \\ 
\end{equation}


% \noindent Practically, the prompt, e.g., 5-way-1-shot, is given as follows: 
% \begin{center}
% \begin{minipage}{0.85\linewidth}
% \footnotesize
% \ttfamily
% <Image: $x_{1,1}^s$> \\
% What is this? $c_1$ (option 1). \\
% ... \\
% <Image: $x_{5,1}^s$> \\
% What is this? $c_5$ (option 5). \\
% <Image: $x^q$> \\
% So what is this? Choose one of the following options: \\
% 1. $c_1$; ...; 5. $c_5$
% \end{minipage}
% \end{center}



\noindent The model is expected to output a class index $\hat{y} \in \{1,\dots,N\}$, which we extract from the generated text via regular expression matching. Full prompt can be found in the top-left of Figure \ref{fig:prompts} (a). We further instruct the model to output the expected answer format. Exact prompts and instruction-following errors are reported in the supplementary material.
% 
% \noindent To predict the final class label $c_{\hat{y}}$, we consider the text output of the model, which should be an index $1...N$ and parse it via regular expression to receive the output index $\hat{y}=\{1...N\}$. We further constrain model outputs to the expected answer format; exact prompts and instruction-following errors are reported in the supplementary material.

\subsection{Decomposed Few-Shot Classification with MLLMs }
\label{subsec:decomposition}
In contrast to in-context learning, we propose to decompose the few-shot classification problem into a set of pairwise comparisons. For each support example and the query image, the model is prompted to determine whether the two images belong to the same class. Given $(\mathcal{S}, x^q)$, we decompose the support set into a set of pairwise prompts: 
\begin{equation}
\mathcal{P} = \bigl\{p_{n,k} \mid n=1,\dots,N,\; k=1,\dots,K\bigr\},
\end{equation}
% \noindent with 
\noindent Each prompt compares the query image with a support example:
\begin{equation}
p_{n,k} =  x^s_{n,k} \oplus x^q \oplus \texttt{Str} \oplus c_n  \\ 
\end{equation}

% \noindent Practically, the prompt is given as follows: 
% \begin{center}
% \begin{minipage}{0.85\linewidth}
% \footnotesize
% \ttfamily
% <Image: $x_{n,k}^s$> \\
% <Image: $x^q$> \\
% The semantic label of the first (support) image is: $c_n$.\\
% Does the second image depict the same class as the support image?\\
% Answer Yes or No.
% \end{minipage}
% \end{center}

All prompts are independently processed by the model. The full prompt can be found in the mid-right of Figure \ref{fig:prompts} (c). For each prompt $p_{n,k}$, the model's output logit for the token \texttt{Yes} is used as the score indicating whether the pair belongs to the same class:
% All prompts are individually processed by the model. 
% We denote by $P(\cdot \mid \mathbf{p_{n,k}})$ the predictive distribution of the MLLM given a multimodal input~$\mathbf{p_{n,k}}$; in practice, this is obtained from the model's token-level log-likelihoods  over the candidate answer tokens. \EK{logits are used not log-likelihoods?}
% Namely, to find the final class index $\hat{y}$, we consider the logit outputs for the token \texttt{Yes} as the score for the respective pair being from the same class :
% \EK{edited this part to make it logit instead of log-likelihood/probabilities - please check.}
\begin{equation}
\label{eq:pairwise}
s_{n,k}^{\mathrm{pair}} = logit(\texttt{Yes} \mid p_{n,k}),
% s_{n,k}^{\mathrm{pair}} = P(\texttt{Yes} \mid p_{n,k}),
\qquad
\hat{y} = \arg\max_{n}\; \frac{1}{K}\sum_{k=1}^{K} s_{n,k}^{\mathrm{pair}},
\end{equation}
where $\hat{y} \in \{1, \dots, N\}$ is the index with the highest averaged pairwise score as the predicted class. This choice is consistent with recent VQA-based scoring approaches such as VQAScore~\cite{lin2024evaluating}, which scores image-text alignment using the \texttt{Yes} token for evaluating text-to-visual generation; in contrast, we score support--query image-pair matches for few-shot image classification.
% \hkc{Prompt exploration in the supplement} \EK{already mentioned in previous section do we need to mention again?}

\subsection{Decomposed Prompting with Domain Information}
\label{subsec:domain}
\input{ECCV_2026/tab/Dinfo_table_main_text}
Decomposed prompting resembles the classical few-shot classification scenario, where a single representation is compared against a set of others. However, MLLMs also offer the ability to further refine this setting by encouraging the model to focus on dataset-specific concepts.
% While decomposed prompting resembles the classical few-shot classification scenario, where one representation is compared against a set of others, MLLMs also offer the ability to further refine the setting, for example by encouraging the model to focus on dataset-specific concepts.
% While the decomposed prompting can be considered close to the classical few-shot classification scenario, where one representation is matched to a set of others, MLLMs also offer to further refine the setting, e.g. to encourage the model to focus on dataset-specific concepts. 
To leverage those capabilities, we replace the generic term \texttt{class} with a domain-appropriate term $D_{\text{info}}$ (e.g., \texttt{pose}, \texttt{texture}, \texttt{species})  
% \EK{Dinfo terms in the supplement, specify that we come up with these terms}
that reflects the concept represented in a given dataset. The full prompt can be found in the bottom-right of Figure \ref{fig:prompts} (e).  The descriptors $D_{\text{info}}$ are inferred for each dataset as shown in Table \ref{tab:dinfo_mapping_main_text}.
%for general cross-domain benchmarks, append brief guidance encouraging semantic rather than stylistic matching.
% \noindent In this case, a single decomposed prompt is given as follows: 
% \begin{center}
% \begin{minipage}{0.85\linewidth}
% \footnotesize
% \ttfamily
% <Image: $x_{n,\cdot}$> \\
% <Image: $x^q$> \\
% The semantic label of the first (support) image is: $c_n$.\\
% Does the second image depict the same $D_{\text{info}}$ as the support image?\\
% Answer Yes or No.
% \end{minipage}
% \end{center}
% \noindent For the anonymized case, the single decomposed prompt is given as follows: 
% \begin{center}
% \begin{minipage}{0.85\linewidth}
% \footnotesize
% \ttfamily
% <Image: $x_{n,k}^s$> \\
% <Image: $x^q$> \\
% Are the two images depicting the same $D_{\text{info}}$?
%  \\
% Answer Yes or No.
% \end{minipage}
% \end{center}
%These modifications preserve the pairwise structure and are applied uniformly within each dataset. 
This grounds each comparison in both visual and textual semantics, allowing the MLLM to leverage its pretrained 
% class-level 
domain-level
knowledge alongside the visual evidence from the support image\footnote{For mini-ImageNet and DomainNet, we use a generic instruction asking the model to focus on the depicted concept rather than domain or texture. See supplement.}. We further provide preliminary evidence in the supplementary material that $D_{\text{info}}$ can be inferred automatically with competitive performance, and we also include example dataset labels to illustrate how $D_{\text{info}}$ captures domain-level information distinct from class labels.
% \hkc{Not sure how to formulate the context label ... we need a table with the domain names for each dataset ... } \YW{We can have the table in supp.}

\subsection{Prompting Without Class Labels }
\label{subsec:labels}
% \EK{is this section too short?}

To isolate the model's ability to learn from visual examples alone, we replace all semantic class names $c_n$ with abstract identifiers
(e.g., \texttt{Class~1}, \dots, \texttt{Class~N}) in both the support demonstrations and the option list.
All other formatting stays identical.
This forces the MLLM to rely on visual similarity rather than leveraging any prior knowledge associated with class names. The full anonymous prompts can be found in the right column of Figure \ref{fig:prompts}.

% \paragraph{In-context Prompt}
% \noindent For the anonymized case... 
% \begin{center}
% \begin{minipage}{0.85\linewidth}
% \footnotesize
% \ttfamily
% <Image: $x_{1,1}^s$> \\
% What is this? Class 1. \\
% ... \\
% <Image: $x_{5,1}^s$> \\
% What is this? Class 5. \\
% <Image: $x^q$> \\
% So what is this? Choose one of the following categories: \\
% Class 1; ...; Class 5
% \end{minipage}
% \end{center}

% Output parsed by regex ... looking for first number/index  

% \paragraph{In-context Prompt}
% \noindent For the anonymized case... \EA{Suggestion to better visually separate the prompts from the rest of the text, definition of this box style is in preamble.tex. With side-by-side figures we also save some space: example beloww}


% \begin{figure}[t]
% \centering

% \begin{minipage}[t]{0.80\linewidth}
% \centering
% \begin{promptbox}
% <Image: $x_{1,1}^s$> \\
% What is this? Class 1. \\
% ... \\
% <Image: $x_{5,1}^s$> \\
% What is this? Class 5. \\
% <Image: $x^q$> \\
% So what is this? Choose one of the following categories: \\
% Class 1; ...; Class 5
% \end{promptbox}
% \subcaption{In-context prompt.}
% \label{fig:prompt-incontext}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.95\linewidth}
% \centering
% \begin{promptbox}
% <Image: $x_{n,k}^s$> \\
% <Image: $x^q$> \\
% Are the two images depicting the same class? \\
% Answer Yes or No.
% \end{promptbox}
% \subcaption{Decomposed pairwise prompt.}
% \label{fig:prompt-pairwise}
% \end{minipage}

% \caption{Prompt formats used in the anonymized case. (a) Standard in-context classification with $N$ labeled supports. (b) Decomposed pairwise verification between each support and the query. \EK{replace with prompt figure}}
% \label{fig:prompt-formats}
% \end{figure}



% \begin{center}
% \begin{minipage}{0.85\linewidth}
% <Image: $x_{1,1}^s$> \\
% What is this? Class 1. \\
% ... \\
% <Image: $x_{5,1}^s$> \\
% What is this? Class 5. \\
% <Image: $x^q$> \\
% So what is this? Choose one of the following categories: \\
% Class 1; ...; Class 5
% \end{minipage}
% \end{center}

% \noindent The model output is parsed by extracting the numeric index appearing after \texttt{Class} in the response.

% \paragraph{Decomposed Pairwise Prompt}
% \noindent For the anonymized case, the single decomposed prompt is given as follows: 

% \begin{center}
% \begin{minipage}{0.85\linewidth}
% \footnotesize
% \ttfamily
% <Image: $x_{n,k}^s$> \\
% <Image: $x^q$> \\
% Are the two images depicting the same class? \\
% Answer Yes or No.
% \end{minipage}
% \end{center}

\subsection{Episode Construction}
\label{subsec:episodes}
% Each episode follows the standard $N$-way $K$-shot protocol~\cite{tipadapter, susx, sav, proker}.
We construct evaluation episodes using the standard $N$-way $K$-shot protocol~\cite{tipadapter, susx, sav, proker}. 
In each episode $e$, an $N$-way label set is sampled, $\mathcal{C} = \{c_1, \dots, c_N\}$, with support set
$\mathcal{S} = \{(x_{n,k}^s, c_n)\}_{n=1,k=1}^{N \times K}$ containing $K$ examples per class, and a single query sample
$\mathcal{Q} = \{(x^q, c_y)\}$.
Given $(\mathcal{S}, x^q)$, the model predicts $\hat{y} \in \{1, \dots, N\}$.
% 
Performance is measured as mean episodic accuracy over a set of evaluation episodes $\mathcal{E}$:
\[
\mathrm{Acc}
=
\frac{1}{|\mathcal{E}|}
\sum_{e \in \mathcal{E}}
\mathbf{1}[\hat{y}_e = y_e].
\]
%We randomly sample $N$ classes and draw $K$ support images per class to form the support set~$\mathcal{S}$. A single query image is then sampled from one of the $N$ classes, with no overlap between query and support images. \NS{should it be in problem formulation?} \YW{I think it can stay since it touches sampling, which we don't have in problem formulation.}
For each dataset, we pre-sample a fixed set of 1000 evaluation episodes using a fixed random seed. 
We verify that cumulative accuracy stabilizes well within 1000 episodes. %, indicating that this number of episodes provides a reliable estimate of model performance. 
% Cumulative accuracy plots with standard error are provided in the supplementary material. 
All evaluation runs are performed on the same set of episodes to ensure fair comparison across models and variants.
% For each dataset, we pre-sample a fixed 1000-episode log at a fixed random seed, as we verify that cumulative accuracy stabilizes well within 1000 episodes. Cumulative accuracy plots with standard error are provided in the supplementary material. All evaluation runs are performed on the same episode log to ensure fair comparison across models and variants. 




% </ ----------------- NEW: Inference Variants: core text --------------/>


==> sec/4_evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}
\subsection{Datasets}
\label{sec:eval_datasets}
We evaluate the proposed technique on a diverse collection of datasets spanning established few-shot benchmarks and novel specialized domains.

\paragraph{Standard benchmarks.}
We evaluate on standard few-shot classification benchmarks following \cite{liu2024, sav, fifty2023context}, including mini-ImageNet~\cite{vinyals2016matching}, a widely used general-purpose few-shot benchmark; CUB~\cite{wah2011caltech}, Aircraft~\cite{maji13fine-grained}, and Dogs~\cite{khosla2011novel}, which test fine-grained visual discrimination within natural categories; UCF101~\cite{soomro2012ucf101} (middle frame of video clip), representing action recognition under a video-to-image transfer. We further remove action images with strong object bias \cite{shvetsova2025unbiasing}. In DomainNet~\cite{Peng_2019_ICCV}, we sample episodes within a single domain at a time, excluding the \textit{real} domain to avoid overlap with the mini-ImageNet domain. 

% \NS{Does DomainNet setup follow the previous paper, or is it new?} \YW{Same setup except we discard the real domain.} \WB{We to add: "See Supplementary Material for more details on the datasets" and in supp. mat we'll add what each dataset is about and how many test/training samples/classes they have.}

\paragraph{Novel datasets.}
We introduce a benchmark suite of six visually distinctive datasets to probe model generalization under stronger domain shift. Namely, we consider the Lego bricks dataset (Lego) \cite{kaggle_lego}, industrial parts (Ind.) \cite{kaggle_industrial}, yoga poses (Yoga) \cite{kaggle_yoga}, ancient Egyptian hieroglyphs (Hiero.) \cite{franken2013automatic}, flying insects (Insect) \cite{kaggle_insect} and Arabic alphabet sign language (Sign) \cite{https://doi.org/10.48550/arxiv.2301.11932}. These cover highly specialized concepts as shown by the particularly low 0-shot recognition performance of pretrained MLLMs. We thus assume that those concepts are only sparsely represented in standard text-image pretraining, making them suitable test cases for evaluating the visual few-shot capabilities of pretrained MLLMs. %More details on the datasets are provided in the supplementary material. 

% \WB{Same comment as above. Especially for these datasets since they are new/uncommon}
% -------------SOTA Table-------------------------

\input{ECCV_2026/tab/SOTA_table}
% -------------------------------------------

\subsection{Experimental Details}

\paragraph{Models.}
We analyze three open-source state-of-the-art MLLMs of comparable scale (7--8B parameters): Qwen2.5-VL-7B-Instruct~\cite{bai2025qwen2}, Qwen3-VL-8B-Instruct~\cite{bai2025qwen3}, 
% its successor with improved visual grounding,
and InternVL3-8B~\cite{zhu2025internvl3}. All models are used in inference-only mode, with token-level 
scores
% log-likelihoods 
extracted directly from output logits as described in Eq.~\eqref{eq:pairwise}.
% \EK{we don't use log-likelihoods?}

\paragraph{SFT Baseline.}
We use supervised fine-tuning (SFT) for Qwen3-VL-8B-Instruct with LoRA \cite{hu2022lora} on the semantic in-context few-shot formulation. The training data consists of 1000 5-way 1-shot episodes sampled from the miniImageNet base classes and the model is trained to output the correct query class. We fine-tune for 3 epochs with LoRA rank 16 and alpha 16, applying LoRA to all non-visual linear modules while keeping the visual modules frozen. Optimization uses a learning rate of ($5\times10^{-5}$), warmup ratio 0.03. The model is then evaluated directly on all target datasets without any further tuning. 

\paragraph{FSL Baselines.}
We compare against a diverse set of few-shot learning baselines. 
CLIP~\cite{lpclip} and SigLIP~\cite{zhai2023sigmoid} are vision-language models that support 0-shot classification via text-image cosine similarity, and few-shot classification via K-nearest neighbour (KNN) search over image embeddings. 
% All CLIP-based methods use a ViT-B/32 backbone. The SigLip model variant is \texttt{base-patch16-224}. 
CLIP uses a ViT-B/32 backbone, while the SigLIP model variant is \texttt{base-patch16-224}. 
DINOv2 \texttt{base} model~\cite{oquab2023dinov2} and I-JEPA (ViT-H/14)~\cite{assran2023self} are vision-only self-supervised models, evaluated via KNN over frozen embeddings. 
Tip-Adapter~\cite{tipadapter} builds a training-free cache model from CLIP features (ViT-B/32).
CAML~\cite{fifty2023context} is a large-scale meta-learning method with a ViT-H encoder pre-trained on Laion-2B \cite{schuhmann2022laion} that performs in-context classification from frozen embeddings. 
ProKeR~\cite{proker} implements training-free kernel regression over pretrained CLIP features (ViT-B/32). 
Finally, SAVs~\cite{sav} directly leverage internal representations of MLLMs for training-free few-shot classification. We implement SAVs on top of Qwen2.5-VL-7B-Instruct, making it the closest baseline to our approach. %Additional implementation details are provided in the supplementary material.

\subsection{Comparison to State-of-the-art}
\label{sec:eval_sota}
% All methods + our best
% with labels vs anonymized ... 

Table~\ref{tab:sota} compares our method against few-shot baselines and recent MLLM-based approaches across standard and novel benchmarks, evaluated under both semantic and anonymized settings. 

\textbf{With semantic labels.}
On standard datasets, 0-shot MLLMs already achieve remarkably strong performance. For example, Qwen3-VL and InternVL3 reach above 90\% average accuracy without any support examples. Interestingly, 1-shot in-context inference often performs worse than 0-shot (e.g., InternVL3 drops from 90.7\% to 72.2\% average; Qwen2.5-VL from 92.2\% to 76.0\%). This indicates that adding support images does not guarantee effective adaptation and may even introduce interference when strong semantic priors dominate.

In contrast, on novel datasets, the trend reverses: 1-shot generally improves over 0-shot. For instance, Qwen3-VL increases from 57.0\% (0-shot avg) to 76.9\% (1-shot avg), suggesting that support examples become more beneficial as pretraining overlap decreases. This highlights the importance of evaluating beyond saturated standard benchmarks.

Across both dataset groups, our decompositional approach consistently outperforms 1-shot inference and matches or surpasses 0-shot performance on standard benchmarks, while substantially outperforming 0-shot performance on novel datasets. Adding dataset-specific domain information further improves results, yielding the best overall averages (e.g., 90.6\% for Qwen3-VL, 88.7\% for Qwen2.5-VL) and establishing new state-of-the-art few-shot performance. 

Compared to the FSL baseline methods, mainly Qwen3-VL models outperform current methods in the simple decomposed setting, while the other two models perform on par. This is expected for standard datasets, given the large-scale pretraining data, but the difference becomes more pronounced for novel datasets, where MLLMs significantly outperform our considered FSL baselines in most cases while remaining on par with the SFT baseline. 

\textbf{Without semantic labels (Anonymous).}
When semantic class names are removed, the performance of in-context 1-shot MLLMs drops dramatically. InternVL3 and Qwen3-VL collapse to near-random prediction (around 23–28\% total average in 5-way classification), revealing a heavy reliance on semantic priors rather than true support–query alignment. Qwen2.5-VL shows slightly more robustness but still degrades substantially.

In stark contrast, the decomposition approach remains highly effective in the anonymized regime. For all three MLLMs, our method restores strong few-shot performance. With Qwen3-VL, it surpasses the SFT baseline by 23.4 points. This shows that structured pairwise inference explicitly enforces visual correspondence and mitigates the semantic dominance.

Interestingly, also in this setting, where MLLMs cannot rely on their textual knowledge, they are able to outperform few-shot baseline methods. We again observe that, also here, the performance difference to the baseline models is smaller on the standard benchmarks, but widens for the novel benchmark setting. This shows that MLLMs might have learned general visual patterns that help them to generalize beyond the training distribution. 

Moreover, in Panel B of Table~\ref{tab:sota}, incorporating \textbf{domain information} leads to consistent overall gains across models and evaluation settings. The improvement is particularly clear on the novel datasets, suggesting that $D_{\text{info}}$ provides useful high-level context about the label space when the classes are less familiar. These results indicate that lightweight domain descriptions can complement decision-based prediction and improve recognition without additional training.

Overall, the results confirm that the proposed decomposed inference framework consistently enables robust few-shot adaptation across both semantic and anonymized settings, achieving state-of-the-art performance.

% \YW{Talk about adding domain info. change words}

% \input{ECCV_2026/tab/SOTA_table_Dinfo}
% \textbf{With domain information.} Table \ref{tab:sota_dinfo}

\subsection{Ablation}
\label{sec:eval_ablation}

\input{ECCV_2026/tab/dec_label_ablation_table}

We ablate three design choices that 
% collectively 
determine the effectiveness of our framework. 
% First, we isolate whether binary decomposition itself or the support–query comparison drives performance gains.

% \YW{Add ablation summary, why do we do ablation. bold and italic, weird}

% \paragraph{Ablation on decomposition and context.} 
% % \YW{Split into 2.}
% % \YW{todo: make connections, make subsubsection }
% In Table \ref{tab:ablation}, we study the effect of injecting the semantic class label of the support image and context-specific knowledge into the prompt of decomposition. Due to the strong presence of prior alignment to canonical class names in MLLMs, we further study the effect of context calibration for the few-shot inference of MLLMs.
% Table~\ref{tab:ablation} isolates the contributions of calibration, decomposition, and context prompting across three MLLMs.

\paragraph{Ablation of Decomposed Prompting.}
First, we analyze whether the performance gains stem from the binary decomposition itself or from the support–query comparison it introduces.
%We first test whether binary prompting alone provides performance gains. 
To this end, we consider a 0-shot decompose variant where no support image is given; the model answers: 
\texttt{“Is this image depicting $c_n$? Yes or No.”} 
In Table~\ref{tab:ablation}, 0-shot decomposition does not improve over standard 0-shot inference and can 
even perform slightly worse
% be slightly worse 
(e.g., Qwen3-VL: 78.2\% → 76.8\%). 
% Thus, 1-shot decomposition gains
This indicates that the gains of 1-shot decomposition do not arise from
% binary formatting, but from support–query comparison.
the binary prompt structure, but from the support-query comparisons.

\paragraph{Ablation on Calibration Effects.}
Second, given that MLLMs exhibit strong language priors, we examine whether the performance of pairwise decomposition just stems from an implicit calibration. %can serve as a simpler alternative to decomposition for reducing prompt bias. 
To this end, we consider an in-context 1-shot inference with calibration. Namely, we apply pointwise mutual information (PMI)-style calibration~\cite{zhao2021calibrate} to reduce option bias introduced by the prompt context.
For each candidate class, we compute the standard prediction given the query image $x^q$ and support set $\mathcal{S}$, and then subtract the score obtained when the query image is replaced by a placeholder text \texttt{“query image is omitted”} while keeping the rest of the prompt unchanged: $P(y|x^q,\mathcal{S})-P(y|\mathcal{S})$. 
As shown in Table~\ref{tab:ablation}, PMI-style calibration mitigates option bias in in-context inference and improves total accuracy (e.g., InternVL3: 62.6\% → 75.0\%; Qwen3-VL: 80.0\% → 86.2\%). 
However, it remains 
% clearly 
inferior to decomposition. Replacing N-way inference with pairwise decomposition consistently yields larger gains (e.g., Qwen3-VL: 86.2\% → 89.2\%), with 
% especially 
particularly great improvements on novel datasets.

% \YW{Refer to method}
% \textbf{Anonymized setting.}
% Without semantic labels, naive 1-shot collapses to near-random prediction (23–29\%) across all considered MLLMs. In contrast, decomposition restores strong performance (e.g., 79–85\% total accuracy), demonstrating that the bottleneck lies in inference structure rather than representation.

% \textbf{Domain prompting.}
% Adding lightweight domain-aware wording (dec.+ctx) further improves results, yielding the best overall performance across models (e.g., 88.5\% total for Qwen2.5-VL and 90.8\% for Qwen3-VL).

% Overall, the ablation shows that while a calibration is able to slightly reduce the prompt bias, the decomposition provides the largest gains, and domain-aware context offers an additional complementary improvement. Together, these components can be considered as a robust framework for the few-shot adaptation of MLLMs under both semantic and anonymized settings.

\paragraph{Evaluation of Logit scoring.}
\input{ECCV_2026/tab/logit_score_table}
Having established decomposition as the key component, we verify that its performance is robust to the choice of logit scoring rule used for ranking.  
Our pairwise inference ranks each support--query pair using the logit score of the \texttt{Yes} token (Eq.~\eqref{eq:pairwise}).
Table~\ref{tab:scoring_rules} compares alternative scoring strategies on Qwen2.5-VL, including: (1) using the model’s generated confidence score output for \texttt{Yes}; (2) minimizing the \texttt{No} logit score: Score(\texttt{No}); (3) a PMI-style correction Score(\texttt{Yes}) - Score(\texttt{No}); (4) the direct \texttt{Yes} logit score.

% the direct \texttt{Yes} logit score: $\text{Score}(\texttt{Yes})$, (ii) a PMI-style correction $\text{Score}(\texttt{Yes}) - \text{Score}(\texttt{No})$, (iii) minimizing the \texttt{No} logit score: $\text{Score}(\texttt{No})$, and (iv) .
% Table~\ref{tab:scoring_rules} compares alternative scoring strategies on Qwen2.5-VL, including: (i) the direct \texttt{Yes} logit score: $\text{Score}(\texttt{Yes})$, (ii) a PMI-style correction $\text{Score}(\texttt{Yes}) - \text{Score}(\texttt{No})$, (iii) , and (iv) using the model’s generated confidence score output for \texttt{Yes}.
The exact prompt used to obtain the confidence score is provided in the supplementary material.
% The exact prompt for confidence score can be found in the supplementary material. 
The three logit-based variants yield nearly identical results across all datasets, confirming 
that the method is robust to the choice of ranking rule.
% robustness to the choice of ranking rule. 
In contrast, using the model's explicit confidence score leads to a substantial drop in accuracy (e.g., 73.3 on mini-ImageNet, 46.9 on Lego), indicating that generative confidence signals are less reliable for fine-grained pairwise matching. We provide further details on scoring in the supplement.

\subsection{5-way 5-shot Analysis}
\label{sec:eval_n_way_kshot}
\input{ECCV_2026/tab/5w5s_table}
We analyze the effect of increasing the number of shots under a fixed 5-way setting. 
The 5-way 5-shot episodes are constructed by extending the corresponding 5-way 1-shot episodes with four additional support samples per class, allowing for a controlled comparison (see also Equation~\ref{eq:pairwise}). Results are reported in Table~\ref{tab:5w_5s} for Yoga, Lego, and Industrial datasets.

While in-context learning benefits from a single support example, its performance deteriorates when moving to 5-shot, suggesting that longer in-context prompts introduce interference rather than improved adaptation.
In contrast, decomposition with $D_{\text{info}}$ consistently improves from 1-shot to 5-shot, achieving the best average accuracy (85.8\%), outperforming the SFT baseline. This behavior highlights a key advantage of decomposition: additional support images contribute positively through independent pairwise aggregation.

% Overall, these results demonstrate that decomposition methods scale effectively in the number of support examples, reinforcing their robustness as a structured few-shot inference framework.


\subsection{N-way 1-shot Analysis}
\label{sec:eval_n_way}
We further analyze the scalability with respect to the number of classes $N \in \{3,5,10,20\}$ under the 1-shot setting. 
In Fig.~\ref{fig:nway_scaling_acc}, In-context inference degrades sharply as $N$ increases. 
While performance is competitive at small $N$, accuracy drops substantially at 10- and 20-way episodes. 
In contrast, our decomposed method remains robust across all $N$, outperforming the SFT baseline. The performance gap widens as the task becomes more challenging, demonstrating that structured pairwise comparison scales more reliably than standard N-way prompting. 
This trend holds consistently across standard, novel, and averaged results, confirming that the improved scalability is not dataset-specific but inherent to the inference structure.

\begin{figure}[t]
  \centering
  \begin{subfigure}[t]{0.49\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/n_way_plot.pdf}
    \caption{$N$-way-1-shot accuracy for comparing \textsc{In-context} and \textsc{Decompose} + domain info performance. We report the average accuracy for standard and novel datasets, as well as for all.}
    \label{fig:nway_scaling_acc}
  \end{subfigure}\hfill
  \begin{subfigure}[t]{0.49\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/n_way_runtime_plot.pdf}
    \caption{$N$-way-1-shot runtime analysis comparing \textsc{In-context} and \textsc{Decompose} + domain info. We report the mean episode latency for single-pass and decomposed batch inference (batch size 64).}
    \label{fig:nway_scaling_runtime}
  \end{subfigure}
  \caption{\textbf{Scaling with $N$-way using Qwen3-VL.} (a) Accuracy comparison between \textsc{In-context} (with and without SFT) and \textsc{Decompose} + domain info. (b) Corresponding runtime analysis under identical decoding and batching settings. $N \in \{3,5,10,20\}$.}
  \label{fig:nway_scaling}
\end{figure}


\subsection{Runtime}
\label{sec:eval_runtime}
The main limitation of decomposition is that it requires access to token logits and incurs $O(N)$ comparisons for an $N$-way problem. Thus, to investigate the computational cost difference, we measure runtime as end-to-end episode latency (ms) in the 1-shot $N$-way setting using Qwen3-VL ($N \in \{3,5,10,20\}$), averaged over 50 episodes per $N$. We compare in-context prompting, which requires one forward pass per episode, and with the proposed pairwise decomposition, which requires $N$ comparisons per episode. All experiments were conducted on a single NVIDIA H100 GPU (80GB) \cite{nvidia2022h100} using \texttt{Bfloat16} precision, deterministic decoding, left padding, CUDA synchronization, and a batch size of 64 for both episodes and generation. We report the mean latency per episode. 

Results in Figure \ref{fig:nway_scaling_runtime} show approximately linear scaling for both single inference and decomposition. The runtime gap is modest at small $N$ but widens at 10--20 way (approximately $1.7\times$ slower at 20-way), reflecting the computational trade-off introduced by structured decomposition. While those numbers reflect the single GPU setting, we argue that, especially for real-world scenarios, settings with larger $N$ or $K$ would most likely aim for a parallelization across multiple GPUs, as all forward paths can be processed independently, which would allow to mitigate longer runtime in those cases if needed. 

 


==> sec/5_conclusion.tex <==
\section{Conclusion}
\label{sec:Conclusion}

We presented a simple yet effective framework for few-shot image classification with multimodal large language models based on \textit{Decompose, Compare, Decide} (DeCoDe). Instead of prompting the model to directly select among class names, our method reformulates classification as binary support--query matching, using the logit of the \texttt{Yes} response as a similarity score aggregated across support examples. This structured inference encourages direct visual comparison and reduces reliance on semantic priors from class labels.

Across both standard and novel benchmarks, the proposed decomposition consistently improves performance over conventional in-context prompting and competitive training-free baselines, achieving state-of-the-art results. The gains are particularly pronounced in the anonymized setting where semantic labels are removed, revealing that structured pairwise comparison more effectively leverages the support set.

These findings suggest a practical inference-time adaptation strategy: users can define new visual categories using a few support images, while the MLLM classifies queries by explicitly comparing them against the provided references without parameter updates.

Beyond the inference method, we introduce a controlled evaluation protocol that disentangles semantic priors from visual adaptation by comparing zero-shot and few-shot regimes with and without semantic labels across diverse datasets. Our results show that standard in-context prompting relies heavily on semantic cues, while the proposed decomposition better captures support adaptation.

% While the method incurs additional inference cost due to pairwise comparisons, it remains simple, model-agnostic, and broadly applicable. These findings highlight the importance of inference structure in unlocking the latent few-shot capabilities of multimodal language models.

% ... We introduce a novel structured inference framework together with a controlled evaluation protocol that systematically disentangles semantic priors from visual adaptation. We explicitly measure the performance gap when semantic labels are removed, directly compare zero-shot and few-shot regimes, and evaluate across both standard and novel datasets and enabling a comprehensive assessment of true support-based adaptation in MLLMs.


\newpage

==> tab/5w5s_table.tex <==

\providecolor{sotaSFTText}{RGB}{130,130,130}
\providecommand{\sft}[1]{\textcolor{sotaSFTText}{#1}}

\begin{table}[t]
\centering
\setlength{\tabcolsep}{4pt}
\small
\begin{tabular}{l cc cc cc |cc}
\toprule
\multicolumn{1}{l}{} &
\multicolumn{8}{c}{\cellcolor{sotaNovelAmber}\scalebox{0.7}{\textbf{Novel Datasets}}} \\[-2pt]
\cmidrule(lr){2-9}
\multirow{2}{*}{Method}
  & \multicolumn{2}{c}{Yoga}
  & \multicolumn{2}{c}{Lego}
  & \multicolumn{2}{c}{Industrial}
  & \multicolumn{2}{c}{Avg} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
  & 5w-1s & 5w-5s & 5w-1s & 5w-5s & 5w-1s & 5w-5s & 5w-1s & 5w-5s \\
\midrule
In-context                    & 74.5 & 45.9 & 66.9 & 43.9 &  80.3 & 60.9 & 73.9 & 50.2 \\
Decompose + $D_{\text{info}}$        & \textbf{88.3} &  \textbf{91.8} &  \textbf{72.9} &  \textbf{80.7} &  \textbf{80.5} & \textbf{85.0} &  \textbf{80.6} &  \textbf{85.8} \\
\sft{SFT baseline}                  & \sft{81.5} & \sft{88.0} & \sft{77.6} & \sft{77.3} &  \sft{78.2} & \sft{82.4} & \sft{79.1} & \sft{82.6} \\
\bottomrule
\end{tabular}
\vspace{2mm}
\caption{Few-shot classification accuracy (\%) on Yoga, Lego, and Industrial datasets under semantic 5-way 1-shot and 5-way 5-shot settings using Qwen3-VL.}
\label{tab:5w_5s}
\end{table}

==> tab/Dinfo_table_main_text.tex <==
% ----------------------------------------------------------------
% Wrapped domain-info table
%
% Preamble packages needed:
%   \usepackage{booktabs,wrapfig}
% ----------------------------------------------------------------

\begin{wraptable}{r}{0.47\linewidth}
\vspace{-3mm}
\centering
\tiny
\setlength{\tabcolsep}{1.2pt}
\renewcommand{\arraystretch}{0.78}

\caption{Mapping of datasets to their domain information text.}
\label{tab:dinfo_mapping_main_text}
\vspace{-1mm}

\begin{tabular}{@{}p{0.56\linewidth}p{0.38\linewidth}@{}}
\toprule
\textbf{Dataset} & \textbf{$D_{\text{info}}$ text} \\
\midrule
mini-ImageNet~\cite{vinyals2016matching} & -- \\
UCF101~\cite{soomro2012ucf101} & action category \\
CUB~\cite{wah2011caltech} & bird species \\
Aircraft~\cite{maji13fine-grained} & aircraft variant \\
Dogs~\cite{khosla2011novel} & dog breed \\
DomainNet~\cite{Peng_2019_ICCV} & -- \\
Lego~\cite{kaggle_lego} & Lego brick type \\
Industrial~\cite{kaggle_industrial} & industrial product \\
Yoga~\cite{kaggle_yoga} & yoga pose \\
Egyptian hieroglyph~\cite{franken2013automatic} & Egyptian hieroglyph \\
Flying insects~\cite{kaggle_insect} & insect species \\
Arabic sign language~\cite{https://doi.org/10.48550/arxiv.2301.11932} & sign language \\
\bottomrule
\end{tabular}

\vspace{-4mm}
\end{wraptable}


==> tab/SOTA_table.tex <==
% ----------------------------------------------------------------
%  sota_table.tex  —  input this file from your ECCV main.tex:
%    \input{sota_table}
%
%  Preamble packages needed:
%    \usepackage{booktabs,colortbl,xcolor,adjustbox,multirow}
% ----------------------------------------------------------------
{
\hypersetup{hidelinks}

\providecolor{sotaStdBlue}{RGB}{210,225,245}
\providecolor{sotaNovelAmber}{RGB}{255,210,160}
\providecolor{sotaSecBlue}{RGB}{235,242,252}
\providecolor{sotaSecOrange}{RGB}{255,245,230}
% \providecolor{sotaModelTint}{RGB}{248,248,248}
% \providecolor{sotaModelGrey}{RGB}{232,232,232}
% \providecolor{sotaPanelGrey}{RGB}{245,242,235}
\providecolor{sotaSFTText}{RGB}{130,130,130}
\providecolor{sotaDinfoTint}{RGB}{255,235,205}
\providecolor{almond}{RGB}{255,235,205}

\providecolor{sotaPanelGrey}{RGB}{235,231,223}  % warm stone, for Panel A/B
\providecolor{sotaModelGrey}{RGB}{242,239,234}  % lighter warm gray, for Semantic/Anonymous sections
\providecolor{sotaModelTint}{RGB}{249,248,246}  % very subtle off-white, for model group rows

\providecommand{\sft}[1]{\textcolor{sotaSFTText}{#1}}
\providecommand{\panelrow}[1]{%
  \specialrule{0.8pt}{3pt}{1pt}
  \multicolumn{17}{l}{\cellcolor{sotaPanelGrey}\textbf{#1}}\\[-1pt]
  \specialrule{0.8pt}{1pt}{2pt}
}

\begin{table*}[!t]
\centering
\begingroup
\setlength{\hfuzz}{15pt}
\resizebox{\textwidth}{!}{%
\fontsize{5.6}{6.7}\selectfont
\setlength{\tabcolsep}{2.1pt}
\renewcommand{\arraystretch}{0.95}
\begin{tabular}{p{1.4cm}@{\hspace{2pt}}p{2.2cm} cccccc|c| cccccc|c|c}
\panelrow{Panel A: Main comparison}
\multicolumn{2}{l}{} &
  \multicolumn{7}{c}{\cellcolor{sotaStdBlue}\textbf{Standard Datasets}} &
  \multicolumn{7}{c}{\cellcolor{sotaNovelAmber}\textbf{Novel Datasets}} & \\[-2pt]
\cmidrule(lr){3-9}\cmidrule(lr){10-16}
\multicolumn{2}{l}{\textbf{Method}}
  & \textbf{mini} & \textbf{UCF} & \textbf{CUB} & \textbf{Air.} & \textbf{Dogs} & \textbf{Dom.} & \textbf{Avg}
  & \textbf{Lego} & \textbf{Ind.} & \textbf{Yoga} & \textbf{Hiero.} & \textbf{Insect} & \textbf{Sign}
  & \textbf{Avg} & \textbf{Total} \\

\midrule

%%--- With labels --------------------------------------------------
\multicolumn{17}{l}{\cellcolor{sotaModelGrey}\textbf{With labels (Semantic)}} \\[-1pt]
\midrule

\multicolumn{17}{l}{\cellcolor{sotaModelTint}\textit{Reported results}} \\
SAVs \cite{sav}               & 1-shot & --   & --   & 98.7 & --   & --   & --   & --   & --   & --   & --   & --   & --   & --   & --   & --  \\
CAML \cite{fifty2023context} & 1-shot & 96.2 & --   & 91.8 & 63.3 & --   & --   & --   & --   & --   & --   & --   & --   & --   & --   & --  \\
GFSL \cite{liu2024}          & 1-shot & 98.2 & --   & 96.6 & 96.6 & 96.7 & --   & --   & --   & --   & --   & --   & --   & --   & --   & --  \\[2pt]

\multicolumn{17}{l}{\cellcolor{sotaModelTint}\textit{Reproduced baselines}} \\
        CLIP \cite{lpclip}                       & 0-shot      & 95.5 & 81.2 & 94.0 & 72.9 & 90.4 & 86.2 & 86.7 & 30.3 & 31.7 & 31.3 & 39.9 & 57.7 & 20.0 & 35.2 & 60.9 \\
        ProKeR \cite{proker}                     & 1-shot      & 98.1 & 89.0 & 94.7 & 73.4 & 92.5 & \textbf{90.3} & 89.3 & 49.7 & 51.7 & 43.2 & 68.1 & 70.3 & 38.2 & 53.5 & 71.4 \\
        SigLip \cite{zhai2023sigmoid}            & 0-shot      & 98.3 & 85.4 & \textbf{97.5} & 79.0 & \textbf{98.7} & 88.2 & 91.5 & 63.0 & 49.4 & \textbf{91.8} & 47.2 & 72.9 & 20.2 & 57.4 & 74.5 \\
        SAVs \cite{sav}                           & 1-shot      & 98.4 & \textbf{94.4} & 96.0 & \textbf{89.4} & 93.1 & 86.2 & \textbf{92.9} & \textbf{68.2} & 57.8 & 62.4 & 64.4 & 80.4 & 28.8 & 60.3 & 76.6 \\
        CAML \cite{fifty2023context}             & 1-shot      & \textbf{98.7} & 90.7 & 95.3 & 86.9 & 94.9 & 81.2 & 91.3 & 62.3 & \textbf{78.0} & 25.2 & \textbf{84.4} & \textbf{95.4} & \textbf{52.3} & \textbf{66.3} & \textbf{78.8} \\[1pt]

\multicolumn{17}{l}{\cellcolor{sotaModelTint}\textit{InternVL3}} \\
                                                 & 0-shot      & \textbf{99.1} & \textbf{95.7} & 89.6 & 73.8 & \textbf{93.7} & \textbf{92.0} & 90.7 & 53.1 & 60.8 & 58.5 & 45.2 & 68.2 & 18.8 & 50.8 & 70.7 \\
                                                 & 1-shot      & 76.2 & 94.8 & 83.2 & 30.3 & 86.6 & 61.8 & 72.2 & 49.0 & 64.9 & 45.2 & 35.6 & 82.4 & 20.0 & 49.5 & 60.8 \\
\rowcolor{almond}                                & 1-shot dec. & 98.4 & 94.5 & \textbf{94.1} & \textbf{75.7} & 92.7 & 89.8 & \textbf{90.9} & \textbf{62.8} & \textbf{75.0} & \textbf{73.6} & \textbf{75.7} & \textbf{89.0} & \textbf{58.7} & \textbf{72.5} & \textbf{81.7} \\[1pt]

\multicolumn{17}{l}{\cellcolor{sotaModelTint}\textit{Qwen2.5-VL}} \\
                                                 & 0-shot      & 97.2 & 93.0 & 96.4 & 89.5 & 91.8 & 85.3 & 92.2 & 50.1 & 42.9 & 50.7 & 43.1 & 80.0 & 20.7 & 47.9 & 70.1 \\
                                                 & 1-shot      & 88.1 & 84.7 & 66.6 & 61.9 & 81.0 & 73.6 & 76.0 & 54.9 & 49.9 & 67.9 & 66.0 & 88.8 & 59.3 & 64.5 & 70.2 \\
\rowcolor{almond}                                & 1-shot dec. & \textbf{98.5} & \textbf{93.7} & \textbf{96.9} & \textbf{94.6} & \textbf{95.8} & \textbf{90.5} & \textbf{95.0} & \textbf{65.5} & \textbf{73.5} & \textbf{80.6} & \textbf{78.1} & \textbf{93.3} & \textbf{67.7} & \textbf{76.5} & \textbf{85.7} \\[1pt]

\multicolumn{17}{l}{\cellcolor{sotaModelTint}\textit{Qwen3-VL}} \\
                                                 & 0-shot      & \textbf{99.1} & 96.6 & 96.5 & 89.1 & \textbf{96.4} & \textbf{92.6} & 95.1 & 63.4 & 62.8 & 66.0 & 48.1 & 80.1 & 21.3 & 57.0 & 76.0 \\
                                                 & 1-shot      & 85.3 & 92.7 & 85.0 & 75.3 & 86.2 & 84.6 & 84.9 & 66.9 & 80.3 & 74.5 & 82.4 & \textbf{89.1} & 68.4 & 76.9 & 80.9 \\
\rowcolor{almond}                                & 1-shot dec. & 98.9 & \textbf{97.3} & \textbf{96.8} & \textbf{92.2} & 96.1 & 91.9 & \textbf{95.5} & \textbf{70.6} & \textbf{81.4} & \textbf{83.4} & \textbf{89.5} & \textbf{89.1} & \textbf{70.6} & \textbf{79.1} & \textbf{87.3} \\
                                                 & \sft{1-shot SFT} & \sft{98.9} & \sft{97.6} & \sft{97.6} & \sft{90.1} & \sft{96.9} & \sft{92.9} & \sft{95.7} & \sft{77.9} & \sft{77.9} & \sft{81.7} & \sft{81.6} & \sft{95.5} & \sft{70.1} & \sft{80.8} & \sft{88.2} \\

\midrule

%%--- Without labels -----------------------------------------------
\multicolumn{17}{l}{\cellcolor{sotaModelGrey}\textbf{Without labels (Anonymous)}} \\[-1pt]
\midrule

\multicolumn{17}{l}{\cellcolor{sotaModelTint}\textit{Reproduced baselines}} \\
        I-JEPA \cite{assran2023self}             & 1-shot      & 76.8 & 75.5 & 53.8 & 32.5 & 79.1 & 39.8 & 59.6 & 45.1 & 42.1 & 60.0 & 68.4 & 45.1 & 31.3 & 48.7 & 54.1 \\
        Tip-A. \cite{tipadapter}                 & 1-shot      & \textbf{97.7} & 82.2 & 93.9 & 70.9 & 90.2 & \textbf{87.0} & \textbf{87.0} & 31.2 & 39.5 & 33.2 & 42.2 & 62.1 & 21.5 & 38.3 & 62.6 \\
        CLIP \cite{lpclip}                       & 1-shot      & 86.5 & 83.0 & 80.6 & 61.0 & 66.7 & 63.9 & 73.6 & 51.3 & 51.5 & 35.3 & 80.4 & 76.8 & 41.5 & 56.1 & 64.9 \\
        DINO \cite{oquab2023dinov2}              & 1-shot      & 93.0 & \textbf{95.2} & \textbf{97.8} & 64.6 & \textbf{95.5} & 74.1 & 86.7 & 65.0 & 73.6 & 52.1 & 85.1 & 66.0 & 40.2 & 63.7 & 75.2 \\
        SigLip \cite{zhai2023sigmoid}            & 1-shot      & 91.3 & 88.6 & 90.4 & \textbf{85.2} & 84.7 & 70.1 & 85.1 & \textbf{70.3} & \textbf{75.7} & \textbf{62.4} & \textbf{87.9} & \textbf{91.0} & \textbf{48.2} & \textbf{72.6} & \textbf{78.8} \\[1pt]

\multicolumn{17}{l}{\cellcolor{sotaModelTint}\textit{InternVL3}} \\
                                                 & 1-shot      & 22.9 & 36.0 & 20.4 & 21.0 & 21.0 & 19.9 & 23.5 & 23.0 & 27.5 & 23.4 & 21.0 & 23.3 & 21.9 & 23.4 & 23.4 \\
\rowcolor{almond}                                & 1-shot dec. & \textbf{94.8} & \textbf{92.8} & \textbf{90.6} & \textbf{70.8} & \textbf{91.4} & \textbf{78.8} & \textbf{86.5} & \textbf{55.4} & \textbf{81.2} & \textbf{51.9} & \textbf{92.1} & \textbf{86.0} & \textbf{76.2} & \textbf{73.8} & \textbf{80.2} \\[1pt]

\multicolumn{17}{l}{\cellcolor{sotaModelTint}\textit{Qwen2.5-VL}} \\
                                                 & 1-shot      & 23.0 & 70.4 & 38.4 & 47.9 & 43.7 & 30.9 & 42.4 & 41.3 & 49.4 & 57.2 & 57.1 & \textbf{88.8} & 68.8 & 60.4 & 51.4 \\
\rowcolor{almond}                                & 1-shot dec. & \textbf{97.0} & \textbf{94.9} & \textbf{96.2} & \textbf{92.8} & \textbf{92.7} & \textbf{82.9} & \textbf{92.8} & \textbf{60.8} & \textbf{73.9} & \textbf{74.6} & \textbf{86.2} & 72.1 & \textbf{76.5} & \textbf{74.0} & \textbf{83.4} \\[1pt]

\multicolumn{17}{l}{\cellcolor{sotaModelTint}\textit{Qwen3-VL}} \\
                                                 & 1-shot      & 21.4 & 26.6 & 38.0 & 39.4 & 27.7 & 20.5 & 28.9 & 25.6 & 31.1 & 21.3 & 30.0 & 23.6 & 28.1 & 26.6 & 27.8 \\
\rowcolor{almond}                                & 1-shot dec. & \textbf{94.9} & \textbf{93.0} & \textbf{87.0} & \textbf{91.1} & \textbf{88.1} & \textbf{79.1} & \textbf{88.9} & \textbf{63.7} & \textbf{81.2} & \textbf{67.5} & \textbf{94.5} & \textbf{33.9} & \textbf{72.6} & \textbf{68.9} & \textbf{78.9} \\
                                                 & \sft{1-shot SFT} & \sft{51.4} & \sft{51.8} & \sft{80.3} & \sft{65.1} & \sft{62.3} & \sft{26.8} & \sft{56.3} & \sft{44.2} & \sft{51.1} & \sft{51.4} & \sft{58.4} & \sft{68.2} & \sft{54.4} & \sft{54.6} & \sft{55.5} \\

\midrule
\panelrow{Panel B: With dataset-specific domain information}

\multicolumn{2}{l}{\textbf{Method}}
  & \textbf{mini} & \textbf{UCF} & \textbf{CUB} & \textbf{Air.} & \textbf{Dogs} & \textbf{Dom.} & \textbf{Avg}
  & \textbf{Lego} & \textbf{Ind.} & \textbf{Yoga} & \textbf{Hiero.} & \textbf{Insect} & \textbf{Sign}
  & \textbf{Avg} & \textbf{Total} \\
\midrule

%%--- Domain info: Semantic -----------------------------------------
\multicolumn{17}{l}{\cellcolor{sotaModelGrey}\textbf{With labels (Semantic)}} \\[-1pt]
\midrule

\multicolumn{17}{l}{\cellcolor{sotaModelTint}\textit{InternVL3}} \\
\rowcolor{almond}        & 1-shot dec.              & \textbf{98.4} & 94.5 & 94.1 & 75.7 & 92.7 & \textbf{89.8} & 90.9 & 62.8 & 75.0 & 73.6 & 75.7 & 89.0 & 58.7 & 72.5 & 81.7 \\
\rowcolor{almond} & 1-shot dec. +$D_{\text{info}}$       & 98.0 & \textbf{94.9} & \textbf{95.1} & \textbf{76.6} & \textbf{93.0} & \textbf{89.8} & \textbf{91.2} & \textbf{64.7} & \textbf{75.3} & \textbf{80.1} & \textbf{77.3} & \textbf{91.8} & \textbf{65.1} & \textbf{75.7} & \textbf{83.5} \\[2pt]

\multicolumn{17}{l}{\cellcolor{sotaModelTint}\textit{Qwen2.5-VL}} \\
\rowcolor{almond}        & 1-shot dec.              & \textbf{98.5} & 93.7 & 96.9 & 94.6 & 95.8 & 90.5 & 95.0 & 65.5 & 73.5 & 80.6 & 78.1 & 93.3 & 67.7 & 76.5 & 85.7 \\
\rowcolor{almond} & 1-shot dec. +$D_{\text{info}}$       & \textbf{98.5} & \textbf{94.3} & \textbf{97.6} & \textbf{95.8} & \textbf{96.5} & \textbf{91.0} & \textbf{95.6} & \textbf{66.4} & \textbf{74.2} & \textbf{84.3} & \textbf{88.1} & \textbf{97.0} & \textbf{80.9} & \textbf{81.8} & \textbf{88.7} \\[2pt]

\multicolumn{17}{l}{\cellcolor{sotaModelTint}\textit{Qwen3-VL}} \\
\rowcolor{almond}        & 1-shot dec.              & 98.9 & \textbf{97.3} & 96.8 & 92.2 & 96.1 & 91.9 & 95.5 & 70.6 & \textbf{81.4} & 83.4 & 89.5 & 89.1 & 70.6 & 79.1 & 87.3 \\
\rowcolor{almond} & 1-shot dec. +$D_{\text{info}}$       & \textbf{99.0} & \textbf{97.3} & \textbf{97.9} & \textbf{93.6} & \textbf{96.6} & \textbf{92.0} & \textbf{96.1} & \textbf{72.9} & 80.5 & \textbf{88.3} & \textbf{90.2} & \textbf{97.4} & \textbf{82.0} & \textbf{85.2} & \textbf{90.6} \\[2pt]

%%--- Domain info: Anonymous ----------------------------------------
\midrule
\multicolumn{17}{l}{\cellcolor{sotaModelGrey}\textbf{Without labels (Anonymous)}} \\[-1pt]
\midrule

\multicolumn{17}{l}{\cellcolor{sotaModelTint}\textit{InternVL3}} \\
\rowcolor{almond}        & 1-shot dec.              & 94.8 & 92.8 & 90.6 & 70.8 & \textbf{91.4} & 78.8 & 86.5 & 55.4 & \textbf{81.2} & 51.9 & \textbf{92.1} & 86.0 & 76.2 & 73.8 & 80.2 \\
\rowcolor{almond} & 1-shot dec. +$D_{\text{info}}$       & \textbf{95.1} & \textbf{95.0} & \textbf{95.3} & \textbf{77.0} & 90.7 & \textbf{80.6} & \textbf{89.0} & \textbf{61.2} & 78.2 & \textbf{84.8} & 90.3 & \textbf{93.8} & \textbf{86.9} & \textbf{82.5} & \textbf{85.7} \\[2pt]

\multicolumn{17}{l}{\cellcolor{sotaModelTint}\textit{Qwen2.5-VL}} \\
\rowcolor{almond}        & 1-shot dec.              & 97.0 & \textbf{94.9} & 96.2 & 92.8 & 92.7 & 82.9 & 92.8 & 60.8 & \textbf{73.9} & 74.6 & \textbf{86.2} & 72.1 & 76.5 & 74.0 & 83.4 \\
\rowcolor{almond} & 1-shot dec. +$D_{\text{info}}$       & \textbf{97.2} & 92.4 & \textbf{97.4} & \textbf{95.2} & \textbf{94.7} & \textbf{84.3} & \textbf{93.5} & \textbf{63.0} & 72.1 & \textbf{84.3} & 83.0 & \textbf{97.5} & \textbf{82.0} & \textbf{80.3} & \textbf{86.9} \\[2pt]

\multicolumn{17}{l}{\cellcolor{sotaModelTint}\textit{Qwen3-VL}} \\
\rowcolor{almond}        & 1-shot dec.              & 94.9 & 93.0 & 87.0 & 91.1 & 88.1 & \textbf{79.1} & 88.9 & 63.7 & \textbf{81.2} & 67.5 & \textbf{94.5} & 33.9 & 72.6 & 68.9 & 78.9 \\
\rowcolor{almond} & 1-shot dec. +$D_{\text{info}}$       & \textbf{95.2} & \textbf{96.6} & \textbf{96.8} & \textbf{92.4} & \textbf{95.4} & 78.7 & \textbf{92.5} & \textbf{68.9} & 80.3 & \textbf{89.6} & 91.2 & \textbf{98.2} & \textbf{86.6} & \textbf{85.8} & \textbf{89.2} \\

\bottomrule
\end{tabular}
}
\endgroup
\vspace{2mm}
\caption{Comparison with state-of-the-art on standard/novel benchmarks for 5-way 1-shot, resp. 0-shot if indicated. Panel A reports the main comparison; Panel B reports the effect of dataset-specific domain information $D_{\text{info}}$. \textit{dec.}~=~decompose and \textit{SFT}~=~supervised fine-tuning. Best results are highlighted \textbf{bold} per subsection. Colored rows mark our method variants.}
\label{tab:sota}
\end{table*}
}

==> tab/baseline_with_dinfo_table.tex <==
\begin{table}[t!]
    \footnotesize
    \centering
    \setlength{\tabcolsep}{3pt}
    \resizebox{0.9\linewidth}{!}{%
    \begin{tabular}{lccc}
    \toprule
    Qwen3-VL-8B & std (mini, cub, dog) & nvl (yoga, hiero., sign) & Avg  \\
    \midrule
    1-shot \textcolor{gray}{(baseline)} & 85.5 & 75.1 & 80.3  \\
    1-shot +$D_{\text{info}}$ & 87.5 & 74.1 & 80.8  \\
    \rowcolor{almond}1-shot dec. \textcolor{gray}{(ours)} & 97.3 & 81.2 & 89.2  \\
    \rowcolor{almond}1-shot dec. +$D_{\text{info}}$ \textcolor{gray}{(ours)} & \textbf{97.8} & \textbf{86.8} & \textbf{92.3} \\
    \multicolumn{4}{l}{\cellcolor{sotaModelGrey}Above: with labels (Semantic); Below: without labels (Anonymous)} \\[-1pt]
    \midrule
    1-shot \textcolor{gray}{(baseline)} & 29.0 & 26.5 & 27.8  \\
    1-shot +$D_{\text{info}}$ & 31.9 & 24.8 & 28.4  \\
    \rowcolor{almond}1-shot dec. \textcolor{gray}{(ours)} & 90.0 & 78.2 & 84.1  \\
    \rowcolor{almond}1-shot dec. +$D_{\text{info}}$ \textcolor{gray}{(ours)} & \textbf{95.8} & \textbf{89.1} & \textbf{92.5} \\
    \bottomrule
    \end{tabular}
    }
    \vspace{2mm}
    \caption{Effect of applying $D_{\text{info}}$ to in-context and decomposed prompting.}
    \label{tab:baseline_Dinfo}
\end{table}

==> tab/cross_model_size.tex <==
\begin{table}[ht]
    \footnotesize
    \centering
    \setlength{\tabcolsep}{3pt}
    \resizebox{0.8\linewidth}{!}{%
    \begin{tabular}{ll|ccc|ccc}
    \toprule
    & & \multicolumn{3}{c}{Qwen3-VL 2B} & \multicolumn{3}{c}{Qwen3-VL 32B} \\
    \toprule
    \multicolumn{2}{l}{Method} & std (m,c,d) & nvl (y,h,s) & Avg  & std (m,c,d) & nvl (y,h,s) & Avg  \\
    \midrule
    %\multirow{3}{*}{2B}
    & 0-shot & \textbf{92.7} & 35.2 & 63.9   & 97.3 & 53.7 & 75.5  \\
    & 1-shot & 85.6 & 60.2 & 72.8   & 91.7 & 81.9 & 86.8  \\
    & \cellcolor{almond}1-shot dec. & \cellcolor{almond}84.8 & \cellcolor{almond}\textbf{68.6} & \cellcolor{almond}\textbf{76.7}  & \cellcolor{almond}\textbf{97.6} & \cellcolor{almond}\textbf{87.3} & \cellcolor{almond}\textbf{92.5}  \\
    \midrule
%    \multirow{3}{*}{32B}
%    & 0-shot & 97.3 & 53.7 & 75.5  \\
%    & 1-shot & 91.7 & 81.9 & 86.8  \\
%    & \cellcolor{almond}1-shot dec. & \cellcolor{almond}\textbf{97.6} & \cellcolor{almond}\textbf{87.3} & \cellcolor{almond}\textbf{92.5}  \\
    \multicolumn{8}{l}{\cellcolor{sotaModelGrey}{Above: with labels (Semantic); Below: without labels (Anonymous)}} \\[-1pt]
    \midrule
    %\multirow{2}{*}{2B}
    & 1-shot & 25.9 & 31.6 & 28.7  & 75.2 & 85.6 & 80.4   \\
    & \cellcolor{almond}1-shot dec. & \cellcolor{almond}\textbf{93.3} & \cellcolor{almond}\textbf{77.5} & \cellcolor{almond}\textbf{85.4}  & \cellcolor{almond}\textbf{86.1} & \cellcolor{almond}\textbf{89.5} & \cellcolor{almond}\textbf{87.8}   \\
    %\midrule
    %\multirow{2}{*}{32B}
    %& 1-shot & 75.2 & 85.6 & 80.4  \\
    %& \cellcolor{almond}1-shot dec. & \cellcolor{almond}\textbf{86.1} & \cellcolor{almond}\textbf{89.5} & \cellcolor{almond}\textbf{87.8}  \\
    \bottomrule
    \end{tabular}
    }
    \vspace{2mm}
    \caption{Evaluation on Qwen3-VL 2B and 32B models}
    \label{tab:model_size}
\end{table}

==> tab/dataset_details.tex <==
\begin{table}[H]
\centering
\begin{tabular}{l|c|c|c|c}
\toprule
\textbf{Dataset} & \textbf{Classes} & \textbf{Total Images} & \textbf{Avg Img/Cls} & \textbf{Eval Classes} \\
\midrule
\multicolumn{5}{l}{\cellcolor{sotaStdBlue}\scalebox{0.8}Standard} \\
mini-ImageNet~\cite{vinyals2016matching}       & 100 & 60,000  & 600   & 20 \\
UCF101~\cite{soomro2012ucf101}             & 101 & 13,320  & 132   & 21 \\
CUB~\cite{wah2011caltech}                & 200 & 11,788  & 59    & 50 \\
Aircraft~\cite{maji13fine-grained}      & 100 & 10,000  & 100   & 100 \\
Dogs~\cite{khosla2011novel}               & 120 & 20,580  & 172   & 30 \\
DomainNet~\cite{Peng_2019_ICCV}          & 345 & 596,006 & 1,728 & 61 \\
\midrule
\multicolumn{5}{l}{\cellcolor{sotaNovelAmber}\scalebox{0.8}Novel} \\
Lego bricks \cite{kaggle_lego}            & 20  & 4,580   & 229    & 20 \\
Industrial \cite{kaggle_industrial}       & 10  & 100,000 & 10,000 & 10 \\
Yoga pose \cite{kaggle_yoga}                  & 107 & 5,991   & 56     & 107 \\
Egyptian hieroglyphs \cite{franken2013automatic}  & 164 & 17,388  & 106    & 164 \\
Flying insects \cite{kaggle_insect}         & 100 & 13,594  & 136    & 100 \\
Arabic sign language \cite{https://doi.org/10.48550/arxiv.2301.11932}   & 31  & 7,856   & 253    & 31 \\
\bottomrule
\end{tabular}
\vspace{2mm}
\caption{Overview of few-shot learning datasets. ``Eval Classes'' is the number of classes used for evaluation (sampled test split).}
\label{tab:dataset_details}
\end{table}

==> tab/dec_label_ablation_table.tex <==
% ----------------------------------------------------------------
%  ablation_table.tex  —  input this file from your ECCV main.tex:
%    \input{ablation_table}
%
%  Preamble packages needed:
%    \usepackage{booktabs,colortbl,xcolor,adjustbox,multirow}
% ----------------------------------------------------------------

\providecolor{sotaStdBlue}{RGB}{210,225,245}
\providecolor{sotaNovelAmber}{RGB}{255, 210, 160}
\providecolor{sotaModelTint}{RGB}{248,248,248}
\providecolor{sotaModelGrey}{RGB}{232,232,232}

\begin{table}[t]
\centering
\begingroup\setlength{\hfuzz}{15pt}\resizebox{\textwidth}{!}{%
\fontsize{7}{9}\selectfont
\setlength{\tabcolsep}{3.5pt}
\renewcommand{\arraystretch}{0.97}
\setlength{\hfuzz}{15pt}
% Cols: [method] [mini CUB Dogs Avg] | [Lego Yoga Hiero. Avg] | Total
\begin{tabular}{p{3.3cm} ccc|c|c ccc|c|c c}
\toprule
\multicolumn{1}{l}{} &
  \multicolumn{4}{c}{\cellcolor{sotaStdBlue}\scalebox{0.8}{\textbf{Standard Datasets}}} & &
  \multicolumn{4}{c}{\cellcolor{sotaNovelAmber}\scalebox{0.8}{\textbf{Novel Datasets}}} & \\[-2pt]
\cmidrule(lr){2-5}\cmidrule(lr){7-10}
\multicolumn{1}{l}{\textbf{Method}}
  & \textbf{mini} & \textbf{CUB} & \textbf{Dogs} & \textbf{Avg}
  & & \textbf{Lego} & \textbf{Yoga} & \textbf{Hiero.} & \textbf{Avg}
  & \textbf{Total} \\
\midrule

%%--- With labels --------------------------------------------------
\multicolumn{11}{l}{\cellcolor{sotaModelGrey}\textbf{With labels (Semantic)}} \\[-1pt]
\midrule

\multicolumn{11}{l}{\cellcolor{sotaModelTint}\textit{InternVL3}} \\
\quad 0-shot                 & \textbf{99.1} & 89.6 & \textbf{93.7} & 94.1 &  & 53.1 & 58.5 & 45.2 & 52.3 & 73.2 \\
\quad 0-shot dec.            & 97.0 & 88.2 & 91.5 & 92.2 &  & 49.4 & 53.9 & 42.4 & 48.6 & 70.4 \\
\quad 1-shot \textcolor{gray}{(baseline)} & 76.2 & 83.2 & 86.6 & 82.0 &  & 49.0 & 45.2 & 35.6 & 43.3 & 62.6 \\
\quad 1-shot calibrated      & 94.0 & \textbf{95.7} & 90.9 & 93.5 &  & \textbf{65.4} & 56.6 & 47.2 & 56.4 & 75.0 \\
\rowcolor{almond}\quad 1-shot dec. \textcolor{gray}{(ours)}           & \underline{98.4} & 94.1 & 92.7 & \underline{95.1} &  & 62.8 & \underline{73.6} & \underline{75.7} & \underline{70.7} & \underline{82.9} \\
\rowcolor{almond}\quad 1-shot dec.+$D_{\text{info}}$ \textcolor{gray}{(ours)}     & 98.0 & \underline{95.1} & \underline{93.0} & \textbf{95.4} &  & \underline{64.7} & \textbf{80.1} & \textbf{77.3} & \textbf{74.0} & \textbf{84.7} \\[2pt]
\multicolumn{11}{l}{\cellcolor{sotaModelTint}\textit{Qwen2.5-VL}} \\
\quad 0-shot                 & 97.2 & 96.4 & 91.8 & 95.1 &  & 50.1 & 50.7 & 43.1 & 48.0 & 71.5 \\
\quad 0-shot dec.            & \underline{97.6} & 96.4 & \underline{96.0} & 96.7 &  & \underline{65.5} & 56.1 & 45.7 & 55.8 & 76.2 \\
\quad 1-shot \textcolor{gray}{(baseline)} & 88.1 & 66.6 & 81.0 & 78.6 &  & 54.9 & 67.9 & 66.0 & 62.9 & 70.8 \\
\quad 1-shot calibrated      & 94.8 & 96.1 & 92.7 & 94.5 &  & 64.1 & 70.7 & 72.7 & 69.2 & 81.8 \\
\rowcolor{almond}\quad 1-shot dec. \textcolor{gray}{(ours)}            & \textbf{98.5} & \underline{96.9} & 95.8 & \underline{97.1} &  & \underline{65.5} & \underline{80.6} & \underline{78.1} & \underline{74.7} & \underline{85.9} \\
\rowcolor{almond}\quad 1-shot dec.+$D_{\text{info}}$ \textcolor{gray}{(ours)}        & \textbf{98.5} & \textbf{97.6} & \textbf{96.5} & \textbf{97.5} &  & \textbf{66.4} & \textbf{84.3} & \textbf{88.1} & \textbf{79.6} & \textbf{88.5} \\[2pt]
\multicolumn{11}{l}{\cellcolor{sotaModelTint}\textit{Qwen3-VL}} \\
\quad 0-shot                 & \textbf{99.1} & 96.5 & \underline{96.4} & \underline{97.3} &  & 63.4 & 66.0 & 48.1 & 59.2 & 78.2 \\
\quad 0-shot dec.            & 96.2 & 96.0 & 95.9 & 96.0 &  & 63.4 & 62.7 & 46.7 & 57.6 & 76.8 \\
\quad 1-shot \textcolor{gray}{(baseline)} & 85.3 & 85.0 & 86.2 & 85.5 &  & 66.9 & 74.5 & 82.4 & 74.6 & 80.0 \\
% \quad 1-shot +$D_{\text{info}}$ & 85.3 & 87.7 & 89.5 & 87.5 &  & 54.7 & 73.7 & 82.5 & 70.3 & 78.9 \\
\quad 1-shot calibrated      & 94.5 & 93.2 & 92.4 & 93.4 &  & \underline{70.9} & 80.0 & 85.8 & 78.9 & 86.2 \\
\rowcolor{almond}\quad 1-shot dec. \textcolor{gray}{(ours)}            & 98.9 & \underline{96.8} & 96.1 & \underline{97.3} &  & 70.6 & \underline{83.4} & \underline{89.5} & \underline{81.2} & \underline{89.2} \\
\rowcolor{almond}\quad 1-shot dec.+$D_{\text{info}}$ \textcolor{gray}{(ours)}        & \underline{99.0} & \textbf{97.9} & \textbf{96.6} & \textbf{97.8} &  & \textbf{72.9} & \textbf{88.3} & \textbf{90.2} & \textbf{83.8} & \textbf{90.8} \\
% \midrule

\bottomrule
\end{tabular}
}\endgroup
\vspace{2mm}
\caption{Ablation on decomposition and context across standard and novel benchmarks (5-way). Top-1 accuracy (\%). \textit{dec.}~=~decompose, \textit{$D_{\text{info}}$}~=~dataset specific domain info. Best and second-best results are highlighted \textbf{bold} and \underline{underlined} per section.}
\label{tab:ablation}
\end{table}

==> tab/dec_label_prompt_variation.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.05}
\begin{tabular}{l|c|c|c|c|c|c|c}
\toprule
\textbf{Prompt} & \textbf{mini} & \textbf{CUB} & \textbf{Dogs} & \textbf{Lego} & \textbf{Yoga} & \textbf{Hiero.} & \textbf{Avg} \\
\midrule
Original prompt    & 99.0 & 97.9 & 96.6 & 72.9 & 88.3 & 90.8 & 90.9 \\
\makecell[l]{Alternative prompt \\ (without support reference)} & 98.7 & 97.3 & 96.3 & 73.1 & 89.5 & 88.8 & 90.6 \\
\bottomrule
\end{tabular}
\vspace{1mm}
\caption{Few-shot classification accuracy (\%) of Qwen3-VL using decomposition with semantic label and domain information under two prompt variants.}
\label{tab:dec_label_prompt_variants}
\end{table}

==> tab/domain_info_ablation.tex <==
{
\hypersetup{hidelinks}

\begin{table}[t!]
\centering
\begingroup
\scriptsize
\setlength{\tabcolsep}{2.8pt}
\renewcommand{\arraystretch}{1.0}
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{l c l c l c}
\toprule
\multicolumn{2}{c}{\textbf{Yoga}} &
\multicolumn{2}{c}{\textbf{Sign}} &
\multicolumn{2}{c}{\textbf{Hiero.}} \\
\cmidrule(lr){1-2}\cmidrule(lr){3-4}\cmidrule(lr){5-6}
\textbf{$D_{\text{info}}$} & \textbf{Acc.} &
\textbf{$D_{\text{info}}$} & \textbf{Acc.} &
\textbf{$D_{\text{info}}$} & \textbf{Acc.} \\
\midrule
class                       & 67.5 & class                         & 72.6 & class                        & \textbf{94.5} \\
\rowcolor{almond} yoga pose \textcolor{gray}{(we use)}          & 89.6 & sign language \textcolor{gray}{(we use)}        & 86.6 & Egyptian hieroglyph \textcolor{gray}{(we use)} & 91.2 \\
pose                        & 89.9 & Arabic sign language          & 66.4 & hieroglyph                   & 93.7 \\
body pose                   & \textbf{90.8} & Arabic alphabet sign language & 59.6 & drawing                      & 94.0 \\
action                      & \underline{90.5} & Arabic sign language alphabet & 57.1 & icon                         & \underline{94.2} \\
\rowcolor{lightgreenrow} yoga stretch \textcolor{gray}{(auto)}         & 88.8 & hand gesture \textcolor{gray}{(auto)}           & \textbf{90.0} & ancient symbol \textcolor{gray}{(auto)}        & 93.5 \\
\rowcolor{lightredrow} kind of flower \textcolor{gray}{(unrelated)}  & 20.6 & kind of flower \textcolor{gray}{(unrelated)}    & 24.0 & kind of flower \textcolor{gray}{(unrelated)}   & 72.9 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\endgroup
\vspace{2mm}
\caption{Effect of different domain information $D_{\text{info}}$ in decomposed prompting (anonymous) with Qwen3-VL on three novel datasets. ``(we use)'' denotes the domain term used in the main paper, while ``(auto)'' denotes a term automatically generated by Qwen3-VL. Best and second-best results are highlighted in \textbf{bold} and \underline{underlined}.}
\label{tab:domain_info_ablation}
\end{table}
}

==> tab/domain_info_mapping.tex <==

\begin{table}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{2.8pt}
\renewcommand{\arraystretch}{1.05}

\begin{tabular}{
>{\raggedright\arraybackslash}p{0.24\linewidth}|
>{\raggedright\arraybackslash}p{0.20\linewidth}|
>{\raggedright\arraybackslash}p{0.43\linewidth}
}
\toprule
\textbf{Dataset} & \textbf{$D_{\text{info}}$ text} & \textbf{Example class labels} \\
\midrule

mini-ImageNet~\cite{vinyals2016matching}
& --
& house finch; triceratops; Tibetan mastiff \\

UCF101~\cite{soomro2012ucf101}
& action category
& ApplyEyeMakeup; BasketballDunk; PlayingGuitar \\

CUB~\cite{wah2011caltech}
& bird species
& Black-footed Albatross; Laysan Albatross; Fish Crow \\

Aircraft~\cite{maji13fine-grained}
& aircraft variant
& Gulfstream V; 727-200; Saab 340 \\

Dogs~\cite{khosla2011novel}
& dog breed
& Chihuahua; Saluki; Pekinese \\

DomainNet~\cite{Peng_2019_ICCV}
& --
& aircraft carrier; cello; lighthouse \\

Lego~\cite{kaggle_lego}
& Lego brick type
& Brick 1$\times$3; Brick 2$\times$2 Slope; Plate 2$\times$4 \\

Industrial~\cite{kaggle_industrial}
& industrial product
& bracket big; engine part cooler square; screw \\

Yoga~\cite{kaggle_yoga}
& yoga pose
& tittibhasana; vajrasana; bakasana \\

Egyptian hieroglyph~\cite{franken2013automatic}
& Egyptian hieroglyph
& road with shrubs; cow with calf; sun disk \\

Flying insects~\cite{kaggle_insect}
& insect species
& Red Cracker; An 88; Danaid Eggfly \\

Arabic sign language~\cite{https://doi.org/10.48550/arxiv.2301.11932}
& sign language
& Alef; Reh; Qaf \\

\bottomrule
\end{tabular}

\vspace{2mm}
\caption{Mapping of datasets to their domain information and example class labels.}
\label{tab:domain_info_mapping}
\end{table}


==> tab/fsar_table.tex <==
\begin{wraptable}[10]{r}{0.46\linewidth}
\vspace{-5mm}
\centering
\scriptsize
\setlength{\tabcolsep}{3.2pt}
\renewcommand{\arraystretch}{0.94}

\caption{Video few-shot results on UCF and Diving48.}
\label{tab:video_fewshot_results}
% \vspace{-1mm}

\begin{tabular}{lcc}
\toprule
\textbf{Setting} & \textbf{UCF101} & \textbf{Diving48} \\
\midrule
\multicolumn{3}{l}{\cellcolor{sotaModelGrey}\textbf{With labels (Semantic)}} \\[-1pt]
\midrule
\multicolumn{3}{l}{\cellcolor{sotaModelTint}\textit{Qwen2.5-VL-7B}} \\
0-shot      & 95.9 & 22.7 \\
1-shot      & 96.8 & 24.7 \\
\rowcolor{almond}
1-shot dec. & 96.4 & 35.5 \\
\bottomrule
\end{tabular}

% \vspace{-3mm}
\end{wraptable}

==> tab/in_contect_prompt_exploration.tex <==
{
\hypersetup{hidelinks}

\providecolor{sotaNovelAmber}{RGB}{255,210,160}
\providecolor{sotaModelGrey}{RGB}{232,232,232}

\begin{table}[t!]
\centering
\small
\begingroup
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.02}
\begin{tabular}{lccc|c}
\toprule
\multicolumn{1}{l}{} &
\multicolumn{4}{c}{\cellcolor{sotaNovelAmber}\scalebox{0.7}{\textbf{Novel Datasets}}} \\
\cmidrule(lr){2-5}
\textbf{Prompt Setting}
& \textbf{Yoga} & \textbf{Hiero.} & \textbf{Sign} & \textbf{Avg.} \\

\midrule
\multicolumn{5}{l}{\cellcolor{sotaModelGrey}\textbf{With semantic label}} \\[-1pt]
\midrule

Standard in-context & 74.5 & \textbf{82.4} & \textbf{68.4} & \textbf{75.1} \\
1. Query first      & \textbf{76.7} & 77.8 & 56.1 & 70.2 \\
3. Images then text & 9.0 & 13.8 & 12.5 & 11.8 \\
4. CoT (Thinking)   & 41.7 & 68.4 & 24.1 & 44.7 \\[2pt]

\midrule
\multicolumn{5}{l}{\cellcolor{sotaModelGrey}\textbf{Anonymous}} \\[-1pt]
\midrule

Standard in-context & 20.3 & 30.0 & 28.1 & 26.1 \\
1. Query first      & \textbf{70.5} & \textbf{80.5} & \textbf{52.5} & \textbf{67.8} \\
2. Visual match     & 18.5 & 12.5 & 15.2 & 15.4 \\
3. Images then text & 5.9 & 20.8 & 8.4 & 11.7 \\
4. CoT (Thinking)   & 9.0 & 47.3 & 2.3 & 19.5 \\

\bottomrule
\end{tabular}
\endgroup
\vspace{2mm}
\caption{In-context prompt exploration on three novel datasets using Qwen3-VL. Standard in-context denotes the interleaved in-context prompting used in the main paper. We experimented with both the semantic and anonymous settings.}
\label{tab:in_context_prompt_exploration}
\end{table}
}

==> tab/instruction_following_score.tex <==
% {
% \hypersetup{hidelinks}

% \providecolor{sotaModelTint}{RGB}{248,248,248}

% \begin{table}[t]
% \centering
% \begingroup
% \small
% \setlength{\tabcolsep}{4.2pt}
% \renewcommand{\arraystretch}{1.03}
% \begin{tabular}{l cc cc cc cc c}
% \toprule
% \textbf{Model}
% & \multicolumn{2}{c}{\textbf{mini}} 
% & \multicolumn{2}{c}{\textbf{CUB}}
% & \multicolumn{2}{c}{\textbf{Yoga}}
% & \multicolumn{2}{c}{\textbf{Lego}}
% & \textbf{Avg.} \\
% \cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
% & \textbf{Sem.} & \textbf{Anon.}
% & \textbf{Sem.} & \textbf{Anon.}
% & \textbf{Sem.} & \textbf{Anon.}
% & \textbf{Sem.} & \textbf{Anon.}
% &  \\
% \midrule

% Qwen3-VL   & 100.0 & 100.0 & 100.0 & 100.0 & 99.9 & 100.0 & 99.1 & 100.0 & 99.9 \\

% InternVL3  & 87.3 & 100.0 & 94.0 & 100.0 & 89.6 & 99.2 & 100.0 & 100.0 & 96.3 \\
% \bottomrule
% \end{tabular}
% \endgroup
% \vspace{2mm}
% \caption{Instruction-following score (\%) of in-context prompting on four datasets for both semantic-label (\textbf{Sem.}) and anonymous (\textbf{Anon.}) setting, computed as $100 -$ instruction-following error rate.}
% \label{tab:instruction_following_score}
% \end{table}
% }

{
\hypersetup{hidelinks}

\begin{table}[t]
\centering
\begingroup
\small
\setlength{\tabcolsep}{4.2pt}
\renewcommand{\arraystretch}{1.03}
\begin{tabular}{l cc cc cc cc c}
\toprule
\multicolumn{1}{c}{} & \multicolumn{9}{c}{\textbf{Instruction-following score (\%) $\uparrow$}} \\
\cmidrule(lr){2-10}
\textbf{Model}
& \multicolumn{2}{c}{\textbf{mini}} 
& \multicolumn{2}{c}{\textbf{CUB}}
& \multicolumn{2}{c}{\textbf{Yoga}}
& \multicolumn{2}{c}{\textbf{Lego}}
& \textbf{Avg.} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
& \textbf{Sem.} & \textbf{Anon.}
& \textbf{Sem.} & \textbf{Anon.}
& \textbf{Sem.} & \textbf{Anon.}
& \textbf{Sem.} & \textbf{Anon.}
&  \\
\midrule
Qwen3-VL  & 100.0 & 100.0 & 100.0 & 100.0 & 99.9 & 100.0 & 99.1 & 100.0 & 99.9 \\
InternVL3 & 87.3  & 100.0 & 94.0  & 100.0 & 89.6 & 99.2  & 100.0 & 100.0 & 96.3 \\
\bottomrule
\end{tabular}
\endgroup
\vspace{2mm}
\caption{Instruction-following score (\%) of in-context prompting on four datasets for both semantic-label (\textbf{Sem.}) and anonymous (\textbf{Anon.}) settings, computed as $100 -$ instruction-following error rate.}
\label{tab:instruction_following_score}
\end{table}
}

==> tab/logit_score_table.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{4pt}
\small
\resizebox{\textwidth}{!}{%
\begin{tabular}{l ccc|c| ccc|c|c}
\toprule
\multicolumn{1}{l}{} &
  \multicolumn{4}{c}{\cellcolor{sotaStdBlue}\scalebox{0.7}{\textbf{Standard Datasets}}} &
  \multicolumn{4}{c}{\cellcolor{sotaNovelAmber}\scalebox{0.7}{\textbf{Novel Datasets}}} & \\[-2pt]
\cmidrule(lr){2-5}\cmidrule(lr){6-9}
Scoring rule & mini & CUB & Dogs & Avg & Lego & Yoga & Hiero. & Avg & Total \\
\midrule
(1) $\arg\max$[Confidence(\texttt{Yes})]                     & 73.3 & 84.6 & 86.6 & 81.5 & 46.9 & 71.2 & 68.2 & 62.1 & 71.8 \\
(2) $\arg\min$[Score(\texttt{No})]                           & 97.0 & 96.1 & 92.9 & 95.3 & 64.1 & 74.4 & 85.7 & 74.7 & 85.0 \\
(3) $\arg\max$[Score(\texttt{Yes}) - Score(\texttt{No})] & 97.1 & 96.2 & 92.6 & 95.3 & 63.9 & 74.4 & 86.1 & 74.8 & 85.1 \\
(4) $\arg\max$[Score(\texttt{Yes})]                             & 97.1 & 96.1 & 92.7 & 95.3 & 64.1 & 74.6 & 86.2 & 75.0 & 85.1 \\
\bottomrule
\end{tabular}
}
\vspace{2mm}
\caption{Comparison of pairwise scoring rules for Qwen2.5-VL in the 5-way 1-shot decomposed setting without semantic labels. All logit-style scoring variants perform nearly identically, confirming the scoring choice (4) of our method.}
\label{tab:scoring_rules}
\vspace{-5mm}
\end{table}

==> tab/variants.tex <==
\begin{table}[t]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|l|l|c|l}
  \toprule
  \textbf{Variant} & \textbf{Paradigm} & \textbf{Label} & \textbf{Domain} & \textbf{Description} \\
  \midrule
  0-shot w. labels           & In-context  & Semantic & \xmark & No support images; only query image and labels given \\
  1-shot w. labels           & In-context  & Semantic & \xmark & Support images with labels given \\
  1-shot w/o labels          & In-context  & Anonymous & \xmark &  Support images with anonymized labels e.g., \texttt{Class~1}, \dots, \texttt{Class~5}  \\
  \midrule
  \rowcolor{almond}\multicolumn{5}{l}{\textit{Ours (Decomposition)}} \\[-1pt]

  1-shot dec. w. labels              & Decompose  & Semantic  & \xmark &  Binary comparisons w. label added to binary question \\
  1-shot dec.+$D_{\text{info}}$ w. labels   & Decompose  & Semantic  & \cmark &  Binary comparisons w. label + Domain-adapted prompt wording \\
  1-shot dec. w/o labels             & Decompose  & Anonymous & \xmark &  Binary comparisons w/o label\\
  1-shot dec.+$D_{\text{info}}$ w/o labels  & Decompose  & Anonymous & \cmark &  Binary comparisons w/o label + Domain-adapted prompt wording \\
  \bottomrule
\end{tabular}%
}
\vspace{2mm}
\caption{Overview of inference variants. Each variant is characterized by its task structure, label naming strategy, and distinguishing mechanism. \textit{dec.}~=~decompose, $D_{\text{info}}$ = domain information.}
\label{tab:variants}
\end{table}


